Clinically Labeled Contrastive Learning for OCT Biomarker Classification

This paper presents a novel positive and negative set selection strategy for contrastive learning of medical images based on labels that can be extracted from clinical data. In the medical field, there exists a variety of labels for data that serve different purposes at different stages of a diagnostic and treatment process. Clinical labels and biomarker labels are two examples. In general, clinical labels are easier to obtain in larger quantities because they are regularly collected during routine clinical care, while biomarker labels require expert analysis and interpretation to obtain. Within the field of ophthalmology, previous work has shown that clinical values exhibit correlations with biomarker structures that manifest within optical coherence tomography (OCT) scans. We exploit this relationship by using the clinical data as pseudo-labels for our data without biomarker labels in order to choose positive and negative instances for training a backbone network with a supervised contrastive loss. In this way, a backbone network learns a representation space that aligns with the clinical data distribution available. Afterwards, we fine-tune the network trained in this manner with the smaller amount of biomarker labeled data with a cross-entropy loss in order to classify these key indicators of disease directly from OCT scans. We also expand on this concept by proposing a method that uses a linear combination of clinical contrastive losses. We benchmark our methods against state of the art self-supervised methods in a novel setting with biomarkers of varying granularity. We show performance improvements by as much as 5\% in total biomarker detection AUROC.

==> Previous/experiments.tex <==



\begin{comment}
\begin{figure*}[t]
\centering
\includegraphics[scale = .5]{images/embedding_cluster.jpg}
\caption{Images from the OLIVES Biomarker dataset labeled by the presence or absence of DME and Fluid IRF were fed into an encoder network trained by using BCVA values as the label. This produced an embedding for each image. These embeddings were visualized using t-SNE \cite{van2008visualizing}  with a single component. The mean and standard deviation for the t-SNE projections for each class are computed and the resulting Gaussian distributions are plotted above. It can be observed that from an encoder trained using BCVA labels with the supervised contrastive loss, we can effectively achieve an embedding space that is separable with respect to biomarkers. }
\label{fig: dme_ebed}
\end{figure*}
\end{comment}


\subsection{Training Details}
Care was taken to ensure that all aspects of the experiments remained the same whether training was done via supervised or self-supervised contrastive learning on the encoder or cross-entropy training on the attached linear classifier. The encoder utilized was kept as a ResNet-18 architecture. The applied augmentations are random resize crop to a size of 224, random horizontal flips, random color jitter, and data normalization to the mean and standard deviation of the respective dataset. The batch size was set at 64. Training was performed for 25 epochs in every setting. A stochastic gradient descent optimizer was used with a learning rate of 1e-3 and momentum of .9. 



\begin{table*}[]
\centering
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multicolumn{8}{c}{OLIVES Clinical Training (Accuracy / F1-Score)}   
\\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{IRF} & \multicolumn{1}{c|}{DME} & \multicolumn{1}{c|}{IRHRF} & \multicolumn{1}{c|}{FAVF} & \multicolumn{1}{c|}{PAVF} & \multicolumn{1}{c|}{MultiLabel} & \multicolumn{1}{c|}{AP} & \multicolumn{1}{c|}{AR} \\\midrule
PCL  \cite{li2020prototypical}              & 76.50\% / .717  & 80.11\% / .761 & 59.1\% /.683 & 76.30\% / .773 & 51.40\% / .165 & .767 & .745 & .6048  \\

SimCLR \cite{chen2020simple}                    & 75.13\% / .715  & 80.61\% / .772 & 59.03\% /.675 & 75.43\% / .761 & 52.69\% / .249 & .7542 & .733 & .614\\
Moco v2 \cite{chen2020improved}                   & 76.00\% / .720      &  82.24\% / .793       & 59.6\% / .692       &  75.00\% / .784      &  52.69\% / .211   & .7709 & .739 & .651 \\ \bottomrule

Eye ID                     & 72.63\% / .674  & 80.2\% / .778   & 58\% / .674    & 74.93\% / .725   & \textbf{65.56}\% / \textbf{.588}  & .767 & .761 & .656\\
CST                        & 75.53\% / .7203   & \textbf{83.06}\% / \textbf{.811}   & 64.3\% / .703  & 76.13\% /.766   & 62.16\% / .509  & .7903 & \textbf{.767} & .675\\
BCVA                       & 74.03\% / .701 & 80.27\% / .770  & 58.8\% / .672  & 77.63\% / .785  & 58.06\% / .418  & .7765 & .749 & .645 \\

BCVA + Eye ID              & 75.2\% / .719  & 79.93\% / .775 & 62.8\% / .691   & \textbf{80.6}\% / \textbf{.806}   & 62.5\% / .504  & \textbf{.806} & .759 & .681\\

BCVA + CST                 &74.5\% / .7019   & 79.69\% / .764  & \textbf{64.43}\% / \textbf{.709}  & 77.06\% / .784   & 63.19\% / .544  & .7875 & .764 & .675\\
CST + Eye ID               & \textbf{76.7}\% / \textbf{.735}  & 81.97\% / .800   & 61.56\% / .693  & 79.2\% / .792   & 62.96\% / .534  & .8012 & .766 & \textbf{.692}\\

BCVA + CST + Eye ID        & 74.86\% / .697 & 79.52\% / .764   & 61.56\% / .681  & 78.66\% / .803  & 59.36\% / .434  & .7939 & .764 & .648\\

 \bottomrule
\end{tabular}
\caption{We show the performance of supervised contrastive training on OLIVES Clinical Dataset and linear layer refinement on OLIVES Biomarker Dataset. MultiLabel refers to the averaged AUROC value during a multi-label classification task. AP and AR refer to average precision and recall across all 5 classes. We evaluate our method against state of the art self-supervised strategies in this table.}
\label{tab:main_table}
\end{table*}



\begin{table}[]
\centering
\begin{tabular}{@{}ccccc@{}}

\toprule
\multicolumn{5}{c}{Evaluation of access to different amounts of biomarker data}                       \\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{25\%} & 
\multicolumn{1}{c|}{50\%} & 
\multicolumn{1}{c|}{75\%} &
\multicolumn{1}{c|}{100\%}\\ \midrule
Supervised                 & .638 & .692  & .687 & .746  \\
Fusion Supervised                 & 0.642 &	0.667 &	0.711&	0.726   \\
PCL  & 0.727 &	0.7487 &	0.7635 &	0.767 \\
SimCLR               &  0.7206 &	0.7297 &	0.7452 &	0.7542  \\
Moco v2               &  0.695&	0.7289&	0.731&	0.7709  \\ \bottomrule
Eye ID               &  0.7134 &	0.7424 &	0.755 &	0.767  \\
CST             &   0.754 &	0.767 &	0.783 &	0.7903 \\
BCVA             &    0.751 &	0.764 &	0.7738 &	0.7765  \\
BCVA + Eye ID               &  \textbf{0.776} &	\textbf{0.788} &	\textbf{0.7985} &	\textbf{0.806}  \\
BCVA + CST              &  0.7506 &	0.7731 &	0.786 &	0.7875 \\
CST + Eye ID                & 0.773 &	0.781 &	0.7919 &	0.8012  \\
BCVA + CST + Eye ID             &   0.7606	 &0.7744 &	0.7858 &	0.7939  \\


 \bottomrule
\end{tabular}
\caption{ We show the performance of different methods when varying the amount of available biomarker training data. We observe the supervised methods are dependent on access to data that isn't so readily available.}
\label{tab:training_split}
\end{table}


\subsubsection{Experiments and Metrics}
During supervised contrastive training, a choice of a single clinical parameter or combination of parameters is chosen to act as labels. For example, in Table \ref{tab:main_table} when the method is specified as BCVA this indicates a supervised contrastive loss $L_{BCVA}$ where BCVA is utilized as the label of interest for the images in the dataset. Additionally, BCVA + CST refers to a linear combination of supervised contrastive losses that can be expressed as $L_{total} = L_{BCVA} + L_{CST}$ where each clinical value respectively  acts as a label for its respective loss. A linear layer is then appended to this trained encoder and trained on the biomarker labels present in the OLIVES Biomarker dataset, consisting of approximately 7,500 images. This linear layer is trained on each biomarker individually and accuracy as well as F1-score in detecting the presence of each individual biomarker is reported. Performance is also evaluated in a multi-label classification setting where the goal is to correctly identify the presence or absence of all 5 biomarkers at the same time. While training in this multi-label setting, a binary cross-entropy loss across the multi-labeled vector was utilized. This is evaluated using averaged area under the receiver operating curve (AUROC) over all 5 classes. This effectively works by computing an AUC for each biomarker and then averaging them. Additionally, we report the average precision and recall across all biomarkers.

\subsubsection{Methods Compared Against}
The setup of interest is compared against a fully supervised and fusion supervised setting as well as state of the art self-supervised contrastive learning frameworks. The fully supervised setting involves standard cross-entropy training of the label of interest without any type of contrastive learning. Fusion supervised is the same as the fully supervised setting except the clinical data for the associated image is appended to the last feature vector before the fully connected layer.  The self-supervised frameworks are SimCLR \cite{chen2020simple}, PCL \cite{li2020prototypical}, and Moco v2 \cite{chen2020improved}. 

\subsection{OLIVES Clinical}
\subsubsection{Comparison with state of the art self-supervised}
We first evaluate the capability of our method to leverage a larger amount of clinical labels for performance improvements on the smaller biomarker subset. This involves supervised contrastive training of the encoder network on the OLIVES Clinical dataset consisting of approximately 60,000 images. Table \ref{tab:main_table} shows that applying our method leads to improvements on classification accuracy of each biomarker individually as well as an improved average AUROC score for detecting all 5 biomarkers concurrently when compared against the state of the art self-supervised algorithms of interest. We can also observe visually how well training on a clinical label performs in creating a separable embedding space for biomarkers through Figure \ref{fig: dme_embed}. This figure was generated by taking a model trained with a supervised contrastive loss on BCVA values and inputting the test set labeled by the biomarkers DME and Intraretinal Fluid. This produces embeddings for each image in the test set. These embeddings are projected into a lower dimensional space with 1-D t-SNE \cite{van2008visualizing}. For each class, the mean and standard deviation on the generated t-SNE values are computed. Using these parameters, we plot a Gaussian curve for each class. It can be observed that the resulting representation can separate between present and absent forms of DME and Fluid IRF without having explicit training for these labels. The Gaussian for each class appears clearly separated between the curve for the biomarker present and absent.  This lends intuition to our point that pre-training with these clinical labels can effectively identify subsets of data that share features that should cluster together and thus act as a good method to choose positives for a contrastive loss. From these results, there are several different analytical points that can act as preliminary explanations for the performance improvements that we observe. 

%This problem is exemplified by the results we observe for the fully supervised setting. Performance is decent for IRF and DME with accuracies of 74.93\% and 82.99\% respectively, but drops drastically for IRHRF, FAVF, and PAVF with performance close to random chance at 50\%. The fully supervised setting isn't able to leverage the unlabeled examples and "overfits" to the easily distinguishable biomarkers without having the robustness necessary to distinguish the more difficult to identify biomarkers.

\subsubsection{Performance of Self-Supervised Algorithms}

Performance of the standard self-supervised methods is comparable to our methods for IRF and DME, but are worse for IRHRF, FAVF, and PAVF.
This difference can be understood through the analysis performed by the authors of \cite{cole2021does}. In this work, the authors showed that the performance gap between contrastive learning and supervised learning increases as the granularity of the task correspondingly increases. They hypothesized that the contrastive loss tends to cluster images based on coarse-visual similarity. This is because the contrastive loss relies on creating positive instances of similar images from augmentations taken from an individual image. In this sense, there is a dependence on the individual image itself to have enough distinguishable features such that a contrast can be created with the negative instances in the loss function. This may not always be the case, especially when it comes to the medical domain where images can be very similar with the exception of small localized regions. We hypothesize that our method is better able to overcome this issue by providing an effective method to identify positive instances that are correlated through having similar clinical metrics. Instead of over-reliance on augmentations from a single image, a more robust set of positive pairs can be found that allows the model to more effectively identify fine-grained features of OCT scans.  This is due to having a wider and more informative set of features to treat as positive instances, thus allowing the model to better identify distinguishing features when using a contrastive loss even for more fine-grained cases.


\subsubsection{Comparison with Supervised}

A major challenge with detecting biomarkers is that they can be associated with small localized changes that exist within the overall OCT scan. IRHRF, FAVF, and PAVF  are examples of biomarkers that fit this criteria. Biomarkers such as IRF and DME are more readily distinguishable as regions of high distortion caused by the presence of fluid within the retina slice. However, since all biomarkers can potentially exist in the image at the same time, this means that the model must be able to resolve small perturbations to distinguish biomarkers simultaneously. This is especially difficult because traditional models are more likely to learn features of the easier to distinguish classes and be unable to identify the more difficult to find classes without sufficient training data~\cite{prabhushankar2020contrastive}. In order to evaluate the impact of access to training data, we take our original training set of 7500 labeled biomarker scans and remove different sized subsets. This is shown in Table \ref{tab:training_split} where each column represents the percentage amount of biomarker training data we restricted each method to have access to. We observe that using our contrastive learning strategy leads to improved performance, regardless of available training data. 

It is interesting to note that the supervised methods, that have access to the biomarker labels during the entirety of training, are significantly worse as the training set is reduced. This shows the dependence that these methods have on a large enough training set because they are unable to leverage representations that may be learnt from the large unlabeled pool of data. The self-supervised methods we compare against are better able to make use of these representations to perform better on the smaller amount of available training data, but are still inferior to our method that integrates clinical labels into the contrastive learning process.
\subsubsection{Performance with respect to individual clinical labels}
Another aspect of the results in Table \ref{tab:main_table} is how well the used clinical labels correspond with the biomarker classification performance. In all cases, the results act as validation to the hypothesis that taking advantage of correlations that exist with certain clinical labels is beneficial for biomarker detection of individual OCT scans. However, from a medical perspective, certain outcomes would intuitively be more likely. For example, for IRF and DME it makes sense that the best performance is associated with using CST values because CST tends to more closely increase or decrease, depending on the severity of IRF and DME. Further analysis showed that combinations of clinical labels with a linear combination of losses such as BCVA + Eye ID and BCVA + CST lead to performance improvements on FAVF, IRHRF, and Multilabel classification. A reason for this is that each clinical value can be thought of being associated with its own distribution of images. By having a linear combination of losses on two clinical values, we are effectively choosing positive instances from closely related, but slightly varying distributions. These distributions are visualized in Figure \ref{fig: clinical_distribution}. It can be observed that because BCVA and CST have different ranges of potential values, as observed along the x-axis of this figure, this means that for any individual value there is a different number of associated eyes and images. Effectively, this means that there is varying diversity with respect to any individual label. This may allow the model to better learn features relating to contrasts that each respective distribution is able to observe. This improves robustness in identifying the more difficult biomarkers which may be the reason for overall improvement in the multi-label classification task.


\subsection{Patient Split Experiments}
In this section, two new training and test sets based on splitting by patient identity are constructed. For the experiments thus far we have evaluated our results on a training and test split based on the eye identity. We show in table \ref{tab:patient_split} that our methods work even in the case where splits between training and testing are made on the basis of different patient identities. It is interesting to note that, depending on the split made, different clinical labels or combinations of clinical labels perform better or worse. This may be due to the fact that each split introduces different distributions of labels that act as positive and negative instances for the contrastive loss as shown by Figure \ref{fig: clinical_distribution}. Certain distributions may be better or worse depending on the split utilized. However, it should be noted that methods that utilized a combined loss such as BCVA + Eye ID were able to maintain consistently high performance across different splits, while there was a much higher variance in methods that used a single clinical label. This indicates that these combined losses have a greater robustness from sampling positive instances from a wider pool of images for each respective loss.

From a medical perspective, the success of our approach across patient and eye splits is indicative of its generalizability. Fully self-supervised approaches are dependent on the data to have enough differentiating features such that augmentations can be used to learn useful features. In this sense, certain groups of patients will potentially be more informative than others, which limits the ability of these approaches to generalize. However, our approach, by choosing positives from a much wider set of data, does not have as strong of a dependence on the features present in any one image. From this perspecitve, there is a greater robustness in regards to patient distributions which corresponds to the better performance across all splits of data.
\begin{table}[]
\centering
\begin{tabular}{@{}cccc@{}}

\toprule
\multicolumn{4}{c}{Patient Split Experiments}                       \\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{Original} & 
\multicolumn{1}{c|}{PS2} & 
\multicolumn{1}{c|}{PS3} \\ \midrule
Supervised & .746 & .7443 & .745\\
Fusion Supervised & .726 & .7699 & .739 \\
PCL & .767 & .724 & .809\\
SimCLR                 & .7542 & .745 & .6177 \\
Moco v2                 & .7709 & .742  & .742 \\ \bottomrule
Eye ID                 & 767 & .7529 & .786 \\
CST                & .7903 & .7669 & .7897\\
BCVA                 & .7765 & .7455 & .8122 \\
BCVA + Eye ID                 & \textbf{.806} & .7802 & .7942 \\
BCVA + CST                 & .7875 & .7559 & .7786 \\
CST + Eye ID                 & .8012 & .7828 & \textbf{.818} \\
BCVA + CST + Eye ID                & .7939 & \textbf{.8032} & .7707 \\


 \bottomrule
\end{tabular}
\caption{ Performance on different training and testing splits, based on the identity of the patient, rather than the identity of the individual eye. This was evaluated with averaged AUC during a multi-label classification task.}
\label{tab:patient_split}
\end{table}

\subsection{Prime Clinical Experiments}
Throughout the paper so far, all experiments have been done on a dataset that was based on combining the Prime and TREX datasets together to form the total OLIVES dataset. However, it is also possible to train the encoder using just the 29000 images in the Prime dataset. There are several interesting analytical points that we can draw from doing this. The first is that the Prime dataset has a wider variety of clinical information that we can potentailly use as a label. In addition to BCVA, CST, and Eye ID that are available across both the Prime and TREX datasets; there are clinical parameters that exist for the Prime dataset specifically such as the type of diabetes of the patient, the diabetic retinopathy severity score (DRSS), and various demographic information. We report the performance of our methodology while leveraging each of these clinical labels in Table \ref{tab:prime}. It can be observed that CST and BCVA out-perform all other methods, but there are certain modalities that perform better than the self-supervised baselines. This includes leakage index and the number of years with diabetes. A possible reason for this is that Prime alone has fewer images as well as less image diversity compared to the original Prime + TREX dataset that we utilized. For this reason, it is not fair to do a direct comparison between Table \ref{tab:main_table} and Table \ref{tab:prime}. The lesser image diversity is due to Prime patients typically having less severe manifestations of their disease than those in the TREX dataset. As a result, regular self-supervised methods are more constrained in the representations that can be drawn from just taking augmentations to form positive pairs in a contrastive loss. However, the methods we developed using a strategy that involves incorporating clinical information still perform satisfactorily even with the constraints imposed by using the Prime dataset alone.  

\begin{table}[]
\centering
\begin{tabular}{@{}cc@{}}

\toprule
\multicolumn{2}{c}{Prime Experiments}                       \\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{MultiLabel} \\ \midrule
PCL                 & .749\\
SimCLR                & .735 \\
Moco v2             &    .7514\\ \midrule
Leakage Index        &        .7741\\
Diabetes Years      &   .748 \\
Diabetes Type         &       .7040\\
Gender                & .6115 \\
DRSS                 & .7132\\
CST                 & .7750\\
BCVA                & \textbf{.776} \\

 \bottomrule
\end{tabular}
\caption{ Performance based on averaged AUROC after training the encoder using data from just the Prime dataset.}
\label{tab:prime}
\end{table}

==> Previous/introduction_draft3.tex <==



\IEEEPARstart{D}{iabetic} Retinopathy (DR) is the leading cause of cases of irreversible blindness among people aged 20 to 74 years old in the United States \cite{klein1995diabetes}. A study in 2012 \cite{yau2012global} indicated that approximately 93 million people worldwide had DR, 17 million had proliferative DR, 21 million had diabetic macular edema, and 28 million had vision-threatening levels of DR. These numbers have only risen since then and projections indicate that as much as 191 million people could have DR by 2030 with 56.3 million having levels of DR that are vision-threatening \cite{zheng2012worldwide}. All of this has amounted to costs estimated at 493 million dollars, according to a comprehensive study performed in 2004 \cite{rein2006economic}.  

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{images/OCT_Biomarkers.jpg}
\caption{Cross-sectional images of graded biomarkers. Intra-Retinal Hyper-Reflective Foci (IRHRF), indicated by the six white arrows, are areas of hyperreflectivity in the intraretinal layers with or without shadowing of the more posterior retinal layers. Intra-Retinal Fluid (IRF) encompasses the cystic areas of hyporeflectivity. Diabetic Macular Edema (DME) is the apparent swelling and elevation of the macula due to the presence of fluid. A Partially Attached Vitreous Face (PAVF), with an arrow indicating the point of attachment and a Fully Attached Vitreous Face (FAVF). A discussion of these biomarkers can be found at \cite{markan2020novel}.\vspace{-0.5cm}}
\label{fig: examples}
\end{figure}
In order to detect and treat DR, the evaluation of biomarkers of the disease is a necessary step in clinical practice \cite{markan2020novel}. Biomarkers refer to “any substance, structure, or process that can be measured in the body or its products and influence or predict the incidence of outcome or disease \cite{strimbu2010biomarkers}." Biomarkers such as Intraretinal Fluid (IRF), Diabetic Macular Edema (DME), and Intra-Retinal Hyper-Reflective Foci (IRHRF) in Figure \ref{fig: examples} are direct indicators of DR. Other biomarkers such as Partially and Fully Attached Vitreous Face (PAVF and FAVF) are not direct indicators of disease, but detecting them can potentially be used to identify certain complications \cite{johnson2010posterior}. These biomarkers are visible on Optical Coherence Tomography (OCT) scans, as shown in Figure~\ref{fig: examples}. 

Hence, 
Given the importance of such biomarkers, it is natural to invest in the development of machine learning algorithms to automate the detection of key biomarkers directly from OCT scans. Automatic detection of these types of biomarkers has the potential to streamline diagnosis and treatment decisions. However, in order to bring this technology to fruition, acquiring access to large quantities of labeled examples is a necessary step to train any conventional deep learning architecture~\cite{alregib2022explanatory}. Obtaining such dataset is a major bottleneck because labels for medical data are expensive and time-consuming to curate. Even in a clinical setting, the interpretation demands of experts have grown disproportionately relative to available staff. A study from 2015 \cite{mcdonald2015effects} showed that radiologists are tasked with interpreting 16.1 images per minute which have contributed to fatigue, burnout, and an increased error-rate.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{images/intro_volume.jpg}
\caption{Clinical and Biomarker labels associated with a single slice and a volume of OCT scans.\vspace{-0.5cm}}
\label{fig: labels}
\end{figure}

Even though biomarker labels for each OCT scan are hard to obtain, there are other types of measurements that are taken as part of standard visits to the opthamologists. These measurements are for the entire retina and cannot be directly labeled on OCT scans. They are termed 
emph{clinical labels}. This is exemplified by Figure \ref{fig: labels} where, in addition to the traditional biomarker labels that are present within individual slices of OCT scans, there are other clinical labels associated with the entire volume of the retina that is taken during routine care with an ophthalmologist. Identifying information such as the patient identity, type of diabetes, and amount of time with diabetes are all easily obtained as part of a reporting process and can act as indicators for the severity of DR \cite{cha2019eye}. Best Corrected Visual Acuity (BCVA) and Central Subfield Thickness (CST) are both collected as part of standard clinical exam procedures. BCVA is measured from eye exam charts and CST values can be processed directly from values obtained from an OCT machine.  Studies such as \cite{hannouche2012correlation,sun2014disorganization,murakami2011association,kashani2010retinal} show that these measured clinical labels can act as indicators of structural changes that manifest themselves in OCT scans as well as the severity of DR associated with the patient. Visually these correlations can be observed from Figure \ref{fig: bcva} where OCT scans with the same BCVA values exhibit more in common structural characteristics  than scans with different BCVA values. This indicates that the clinical labels, that are collected in abundance during standard clinical practice, exhibit non-trivial relationships with key biomarkers of DR.

\begin{comment}
From the above discussion, the main challenges we aim to address are that fine-grained biomarker labels are difficult to obtain and that it isn't so clear how to utilize the correlations present in the larger corpus of clinically labeled data to improve biomarker detection performance. In this paper, we address this challenge by using a contrastive learning approach \cite{le2020contrastive} that incorporates clinical labels into the positive and negative pair selection process.
\end{comment}

Hence, we make use of this relationship to detect biomarkers in OCT scans by utilizing the abundantly present clinical labels. In this paper, we utilize the correlations present in the larger corpus of clinically labeled data to improve biomarker detection performance. In particular, we address this detection by using a contrastive learning approach \cite{le2020contrastive} that incorporates clinical labels into the deep learning framework. Contrastive learning is a methodology that functions by creating a representation space by minimizing the distance between positive pairs and maximizing the distance between negative pairs of images. Traditional contrastive learning approaches, such as \cite{chen2020simple}, generate positive pairs from augmentations of a single image and treat all other images in the batch as the negative pairs. However, from a medical imaging point of view, arbitrary augmentations like in~\cite{chen2020simple} have the potential to occlude the small localized regions where biomarkers may be present. The authors in~\cite{khosla2020supervised} choose positive pairs within the same class label and negative pairs are from all other classes. However, in our setting, the supervised biomarker-labeled data is insufficient to perform supervised contrastive learning due to the relatively scarce amount of available data. Hence, state of the art contrastive learning techniques that perform well on natural image datasets may not be applicable to medical data as will be illustrated in this paper. 

\begin{comment}
In order to improve upon these issues, choosing positive pairs of instances from strategies beyond just augmentations presents a promising path. This is the premise behind the supervised contrastive loss \cite{khosla2020supervised} where similar pairs are chosen from augmented images with the same class label and dissimilar pairs are chosen from images of all other classes. 
\end{comment}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{images/bcva_comparison.jpg}
\caption{Examples images from OCT Scans of pairs of images with same BCVA value and different BCVA values across different patients. It can be observed the same BCVA values corresponded with images that have more structural features in common.\vspace{-0.5cm}}
\label{fig: bcva}
\end{figure}

In this paper, we perform supervised contrastive learning by utilizing clinical labels to discriminate between positive and negative pairs of images. This will allow the model to learn a representation space that can effectively separate embeddings of OCT scans into semantically interpretable groups by enforcing images with similar BCVA values, CST values, or images from the same eye be close to each other, in the representation space. These representations will then be utilized to train a linear classifier utilizing a much smaller subset of biomarker labels. As a result, the model will be able to utilize the larger pool of clinical labels in order to better learn how to classify specific biomarkers. The contributions of this paper are four fold as follows:

\begin{enumerate}
  \item We utilize clinical labels associated with OCT scans to train an effective supervised contrastive learning framework.
  
  \item We demonstrate that our strategy outperforms traditional approaches that use direct supervision on biomarker labels as well as state of the art self-supervised strategies.
  
  \item We perform our analysis on a novel OCT dataset containing both fine-grained biomarker labels as well as comprehensive clinical information. 
  
  \item We perform comprehensive studies on clinical label usage and their effects on biomarker identification.
\end{enumerate}



==> Previous/introduction_draft4.tex <==



\IEEEPARstart{B}{iomarkers} refer to “any substance, structure, or process that can be measured in the body or its products and influence or predict the incidence of outcome or disease \cite{strimbu2010biomarkers}." In order to detect and treat disease, the evaluation of biomarkers is a necessary step in any clinical practice \cite{markan2020novel}. However, interpretation of biomarkers from imaging data is a time-consuming and expensive process. In a clinical setting, the interpretation demands of experts have grown disproportionately relative to available staff. A study from 2015 \cite{mcdonald2015effects} showed that radiologists are tasked with interpreting 16.1 images per minute which have contributed to fatigue, burnout, and an increased error-rate. Given the importance of biomarkers and their difficulty in acquisition, it is natural to invest in the development of machine learning algorithms to automate the detection of key biomarkers directly from their associated imaging modality. Accomplishing this goal would assist clinical practitioners in making better treatment decisions with the goal of arriving at more favorable outcomes for their patients. In order to bring this technology to fruition, acquiring access to large quantities of labeled examples is a necessary step to train any conventional deep learning architecture~\cite{alregib2022explanatory}. Obtaining such a dataset is a major bottleneck because labels for medical data are expensive and time-consuming to curate due to the aforementioned difficulties with interpretation. Even though biomarker labels are hard to obtain, there are other types of measurements that are taken as part of standard visits to the clinical practitioner that are typically easier to obtain in large quantities. They are termed \emph{clinical labels}. In this paper, we utilize the correlations present in the larger corpus of clinically labeled data to improve biomarker detection performance for indicators of the disease Diabetic Retinopathy (DR) within the setting of Optical Coherence Tomography (OCT) scans. 

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{images/OCT_Biomarkers.jpg}
\caption{Cross-sectional images of graded biomarkers. Intra-Retinal Hyper-Reflective Foci (IRHRF), indicated by the six white arrows, are areas of hyperreflectivity in the intraretinal layers with or without shadowing of the more posterior retinal layers. Intra-Retinal Fluid (IRF) encompasses the cystic areas of hyporeflectivity. Diabetic Macular Edema (DME) is the apparent swelling and elevation of the macula due to the presence of fluid. A Partially Attached Vitreous Face (PAVF), with an arrow indicating the point of attachment and a Fully Attached Vitreous Face (FAVF). A discussion of these biomarkers can be found at \cite{markan2020novel}.\vspace{-0.5cm}}
\label{fig: examples}
\end{figure}

Biomarkers such as Intraretinal Fluid (IRF), Diabetic Macular Edema (DME), and Intra-Retinal Hyper-Reflective Foci (IRHRF) in Figure \ref{fig: examples} are direct indicators of (DR). Other biomarkers such as Partially and Fully Attached Vitreous Face (PAVF and FAVF) are not direct indicators of disease, but detecting them can potentially be used to identify certain complications \cite{johnson2010posterior}. These specific biomarkers are visible on OCT scans, as shown in Figure~\ref{fig: examples}. Even though acquiring access to these biomarkers are difficult, there are oftentimes associated clinical labels taken during routine care with an ophthalmologist. Identifying information such as the patient identity, type of diabetes, and amount of time with diabetes are all easily obtained as part of a reporting process \cite{cha2019eye}. Best Corrected Visual Acuity (BCVA) and Central Subfield Thickness (CST) are both collected as part of standard clinical exam procedures. BCVA is measured from eye exam charts and CST values can be processed directly from values obtained from an OCT machine. Visually it can be be observed from Figure \ref{fig: bcva} that OCT scans with the same BCVA values exhibit more common structural characteristics  than scans with different BCVA values. Studies such as \cite{hannouche2012correlation,sun2014disorganization,murakami2011association,kashani2010retinal} confirm that these measured clinical labels can act as indicators of structural changes that manifest themselves in OCT scans as well as the severity of DR associated with the patient. These works indicate that the clinical labels that are collected in abundance during standard clinical practice exhibit non-trivial relationships with key biomarkers of DR.

 \begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{images/intro_volume.jpg}
\caption{Clinical and Biomarker labels associated with a single slice and a volume of OCT scans.\vspace{-0.5cm}}
\label{fig: labels}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{images/bcva_comparison.jpg}
\caption{Examples images from OCT Scans of pairs of images with same BCVA value and different BCVA values across different patients. It can be observed the same BCVA values corresponded with images that have more structural features in common.\vspace{-0.5cm}}
\label{fig: bcva}
\end{figure}


We make use of these correlations that exist in clinical data in order to improve biomarker detection performance. In particular, we address this detection by using a contrastive learning approach \cite{le2020contrastive} that incorporates clinical labels into the deep learning framework. Contrastive learning is a methodology that functions by creating a representation space by minimizing the distance between positive pairs and maximizing the distance between negative pairs of images. Traditional contrastive learning approaches, such as \cite{chen2020simple}, generate positive pairs from augmentations of a single image and treat all other images in the batch as the negative pairs. However, from a medical imaging point of view, arbitrary augmentations, like in~\cite{chen2020simple}, have the potential to occlude the small localized regions where biomarkers may be present. The authors in~\cite{khosla2020supervised} choose positive pairs within the same class label and negative pairs are from all other classes. However, in our setting, the supervised biomarker-labeled data is insufficient to perform supervised contrastive learning due to the relatively scarce amount of available data. Hence, state of the art contrastive learning techniques that perform well on natural image datasets may not be applicable to medical data as will be illustrated in this paper. 

In this paper, we perform supervised contrastive learning by utilizing clinical labels to discriminate between positive and negative pairs of images. This will allow the model to learn a representation space that can effectively separate embeddings of OCT scans into semantically interpretable groups by enforcing images with similar BCVA values, CST values, or images from the same eye be close to each other, in the representation space. These representations will then be utilized to train a linear classifier utilizing a much smaller subset of biomarker labels. As a result, the model will be able to utilize the larger pool of clinical labels in order to better learn how to classify specific biomarkers. The contributions of this paper are four fold as follows:

\begin{enumerate}
  \item We utilize clinical labels associated with OCT scans to train an effective supervised contrastive learning framework.
  
  \item We demonstrate that our strategy outperforms traditional approaches that use direct supervision on biomarker labels as well as state of the art self-supervised strategies.
  
  \item We perform our analysis on a novel OCT dataset containing both fine-grained biomarker labels as well as comprehensive clinical information. 
  
  \item We perform comprehensive studies on clinical label usage and their effects on biomarker identification.
\end{enumerate}

==> Previous/methodology2.tex <==




Since the methodology is inspired by different amounts of available clinical and biomarker labels in data, a thorough understanding of the datasets used in this paper is needed before diving into technical details.
\begin{comment}
\begin{figure*}[t]
\centering
\includegraphics[scale = .5]{images/distribution_graphs.jpg}
\caption{Distribution of CST and BCVA labels in the OLIVES dataset based on number of eyes associated with each clinical value.}
\label{fig: clinical_distribution}
\end{figure*}
\end{comment}
\subsection{Datasets}
The Prime and TREX-DME studies provide a wealth of clinical information as part of their respective trials. In addition to this information provided by the studies, a trained grader performed interpretation on OCT scans for the presence of 20 different biomarkers including: Intra-Retinal Hyper-Reflective Foci (IRHRF), Partially Attached Vitreous Face (PAVF), Fully Attached Vitreous Face (FAVF), Intra-Retinal Fluid (IRF), and Diffuse Retinal Thickening or Macular Edema (DRT/ME). The trained grader was blinded to clinical information whilst grading each of 49 horizontal SD-OCT B-scans of both the first and last study visit for each individual eye. This results in a subset of both studies now having just clinical labels and a smaller subset having both clincial and biomarker labels as observed in table \ref{tab: data_all}.  Open adjudication was done with an experienced retina specialist for difficult cases.

In addition to the clinical information
provided by the original studies, we introduced explicit biomarker labels to a subset of this data. A trained grader performed interpretation
on OCT scans for the presence of 20 different biomarkers. The trained grader was blinded
to clinical information whilst grading each of the 49 horizontal
SD-OCT B-scans of both the first and last study visit for
each individual eye. Open adjudication was done with an
experienced retina specialist for difficult cases.

As a result, for each OCT scan labeled for biomarkers, there exists a one-hot vector indicating the presence or absence of 20 different biomarkers. Of these 20 biomarkers, 4 do not appear within the dataset which effectively means that 16 are present within the dataset. Not all of these 16 biomarkers exist in sufficiently balanced quantities to train a model to identify their presence or absence within an image. Hence, we use Intraretinal Hyperreflective Foci (IRHRF), Partially Attached Vitreous Face (PAVF), Fully Attached Vitreous Face (FAVF), Intraretinal Fluid (IRF), and Diffuse Retinal Thickening or Diabetic Macular Edema (DRT/ME) as the biomarkers that are studied in this paper.  It should be noted that because Prime and TREX DME are different studies with different intended outcomes, this results in each having different types of clinical information. When combining the datasets together, we only focus on the clinical data that is commonly held by both datasets: BCVA, CST, and Eye ID. This overall dataset is known as the Ophthalmic Labels for
Investigating Visual Eye Semantics (OLIVES) dataset and further details can be found at \cite{prabhushankar2022olives}. For convenience we will refer to the data subset with biomarker and clinical labels as OLIVES Biomarker and the larger subset with clinical data as OLIVES Clinical. We present the manifestation of distributions within the OLIVES dataset for the clinical values of BCVA and CST in Figure \ref{fig: clinical_distribution}. It can be observed that the distribution of BCVA and CST values across eyes and image quantities isn't noticeably biased towards any specific value. Instead, for each value, there is diversity in terms of the number of different eyes and number of images.  In the case of biomarker information, this distribution problem doesn't exist because the identified images to be labeled are labeled in the same binary vector fashion for both datasets. All of the data label availability with regards to clinical and biomarker information are summarized in table \ref{tab: data_all}. 



\begin{figure*}[ht]
\centering
\includegraphics[scale = .4]{images/methodology.jpg}
\caption{ Overview of Experimental Setup. 1) Supervised contrastive learning is performed on the larger amount of available clinical data provided in OLIVES Clinical. 2) This trained encoder then has its weights frozen and a linear classifier is trained utilizing the smaller amount of data from the OLIVES Biomarker dataset.}
\label{fig: supcon}
\end{figure*}

Together the Prime and TREX studies have provided data from 96 unique eyes from 87 unique patients. We take 10 unique eyes from the Prime dataset and 10 unique eyes from the TREX dataset and use the data from these 20 eyes to create the test set. The remaining 76 eyes are utilized for training in all experiments. Since the objective is to evaluate the model's performance in identifying each biomarker individually, a test set for each biomarker is created. This is done by randomly sampling 500 images with the biomarker present and 500 images with the biomarker absent from the data associated with the test eyes. In this way, we ensure that the test set for each individual biomarker is balanced.

In the case of nine patients there exists data for the left and right eye. This leads to questions as to whether this may potentially bias any experiments that are performed by having both in the dataset. However, in the original Prime and TREX DME studies, each eye is treated as independent from every other eye and different experimental settings are applied to each. Consequently, random splits of experiments were made on the basis of the eye identity, rather than the patient identity. This also means that data is recorded for individual eyes, rather than individual patients. So as to align with the setup of the original studies, we make our train and test split on the basis of the eye identity. Ablation studies later in the paper show that our methods perform comparably even if we were to make the split based solely on patient identity.

\subsection{Overall Framework}
The overall block diagram of the proposed method is summarized in Figure \ref{fig: supcon}. Within the OLIVES Clinical dataset, each individual image is associated with the clinical values BCVA, CST, and Eye ID that are taken during the original patient visit. For each experiment, we first choose one of these clinical values to act as a label for each image in the dataset. 

Given an input batch of data, $(x_{k}$, and clinical label, $(y_{k}$, pairs $(x_{k},y_{k})_{k=1,...,N}$, we perform augmentations on the batch twice in order to get two copies of the original batch with $2N$ images and clinical labels. These augmentations are random resize crop to a size of 224, random horizontal flips, random color jitter, and data normalization. These are sensible from a medical perspective because they don't disrupt the general structure of the image.
This process produces a larger set $(x_{l},y_{l})_{l=1,...,2N}$ that consists of two versions of each image that differ only due to the random nature of the applied augmentation. Thus, for every image $x_{k}$ and clinical label $y_{k}$ there exists two views of the image $x_{2k}$ and $x_{2k-1}$ and two copies of the clinical labels that are equivalent to each other: $y_{2k-1} = y_{2k} = y_{k}$.

From this point, we perform the first step in Figure \ref{fig: supcon}, where supervised contrastive learning is performed on the identified clinical label. The clinically labeled augmented batch is forward-propagated through an encoder network $f(\cdot)$ that we set to be the ResNet-18 architecture \cite{he2016deep}. This results in a 512-dimensional vector $r_{i}$ that is sent through a projection network $G(\cdot)$, which further compresses the representation to a 128-dimensional embedding vector $z_{i}$. $G(\cdot)$ is chosen to be a multi-layer perceptron network with a single hidden layer. This projection network is utilized only to reduce the dimensionality of the embedding before computing the loss and is discarded after training. A supervised contrastive loss is performed on the output of the projection network in order to train the encoder network. This can be understood by the example shown at the bottom of Figure \ref{fig: supcon}. In this case, embeddings with the same BCVA label are enforced to be projected closer to each other while embeddings with differing BCVA labels are projected away from each other.  Our introduced clinical supervised contrastive loss process can be understood by:
$$
    L_{supcon_{clinical}} = \sum_{i\in{I}} \frac{-1}{|C(i)|}\sum_{c\in{C(i)}}log\frac{exp(z_{i}\cdot z_{c}/\tau)}{\sum_{a\in{A(i)}}exp(z_{i}\cdot z_{a}/\tau)}
$$
where $i$ is the index for the image of interest $x_{i}$.
All positives $c$ for image $x_{i}$ are obtained from the set $C(i)$ and all positive and negative instances $a$ are obtained from the set $A(i)$. Every element $c$ of $C(i)$ represents all other images in the batch with the same clinical label $c$ as the image of interest $x_{i}$. Additionally, $z_{i}$ is the embedding for the image of interest, $z_{c}$ represents the embedding for the clinical positives, and $z_{a}$ represents the embeddings for all positive and negative instances in the set $A(i)$. $\tau$ is a temperature scaling parameter that is set to .07 for all experiments.  The loss function operates in the embedding space where the goal is to maximize the cosine similarity between embedding $z_{i}$ and its set of clinical positives $z_{c}$. It should be explicitly stated that the set $C(i)$ can represent any clinical label of interest. Throughout the rest of the paper we will use certain conventions to make the choice of clinical label in the loss transparent. For example, a loss represented as $L_{BCVA}$ indicates a supervised contrastive loss where BCVA is utilized as the clinical label of interest. Furthermore, it is also possible to create an overall loss that is a linear combination of several losses on different clinical labels. This can be represented by $L_{total} = L_{BCVA} + L_{CST}$ where each clinical value respectively acts as a label for its respective loss.

After training the encoder with  clinical supervised contrastive loss, we move to the second step in Figure \ref{fig: supcon} where the weights of the encoder are frozen and a linear layer is appended to the output of the encoder. This setup is trained on the OLIVES Biomarker dataset after choosing the biomarker we wish to train for. This linear layer is trained using cross-entropy loss to distinguish between the presence or absence of the biomarker of interest in the OCT scan. In this way, we leverage knowledge learnt from training on clinical labels to improve performance on classifying biomarkers. In the example detailed in part 2 of Figure \ref{fig: supcon}, the biomarker of interest is chosen to be DME and the input images to the network are labeled by the presence or absence of DME. The previously trained encoder with the supervised contrastive loss on the BCVA label from step 1 produces the representation for the input and this representation is fine-tuned with the linear layer to distinguish whether or not DME is present. 


%In addition to performing supervised contrastive learning on individual clinical labels, there are various other ways to utilize this setup to improve on the existing representation space. For example, if $L_{BCVA}$ is the loss for performing supervised contrastive learning when using BCVA values as labels for the OCT scans, then it should be possible to create an overall loss that is a linear combination of losses based on multiple clinical labels. This could include a loss like $ L = \alpha L_{BCVA} + \beta L_{CST}$ where $L_{CST}$ is a supervised contrastive loss from treating the CST values as labels and $L_{BCVA}$ being a loss from treating the BCVA values as labels for the images in the dataset. It is also possible to utilize the biomarkers as part of a loss function with the clinical labels. In this case, we would use the Prime + TREX Biomarker dataset and perform supervised contrastive learning on a biomarker, such as DME, alongside a clinical label, such as BCVA. Such a loss function could look like $ L = \alpha L_{BCVA} + \beta L_{DME}$ where $L_{DME}$ is a supervised contrastive loss from treating the presence or absence of DME as the label of interest. The rest of this paper will be a comprehensive analysis of these experiments on clinical and biomarker labels within different settings and scenarios.

==> Previous/related_works.tex <==


In this section, we summarize the related work based on six relevant categories: incorporating clinical data in multi modal learning, deep learning in OCT, standard contrastive learning strategies, contrastive learning with clinical information, supervised contrastive learning, and previous OCT Datasets.

\subsection{Incorporating Clinical Data with Multi-Modal Learning}
A survey of radiologists \cite{boonn2009radiologist} showed that access to clinical labels had an impact on the quality of interpretation of images. However, standard deep learning architectures only utilize visual scans without contextualization of other clinical labels. This has motivated research into different ways of incorporating clinical labels into the deep learning framework. One approach that has gained traction is to treat clinical labels as its own feature vector and then fuse this with the features learned from a CNN on associated image data. \cite{xu2016multimodal} showed how combining image features from a cervigram with clinical records such as PH-value, HPV signal strength, and HPV status could be utilized to train a network to diagnose cervical dysplasia. \cite{zhang2019multi} incorporated data from a neurophysical diagnosis with features from MRI and PET scans for Alzheimer's detection. \cite{kharazmi2018feature} combined image information along with skin lesion data such as lesion location, lesion size, and elevation for the task of basal cell carcinoma detection. Similarly, \cite{yap2018multimodal} utilized macroscopic and dermatoscopic data along with patient meta data for improved skin lesion classification. \cite{miled2020predicting} performed a fusion of EMR datasets with various information such as diagnosis, prescriptions, and medical notes for the task of dementia detection. Other works have performed multi-modal fusion between different types of imaging domains. \cite{rajalingam2018multimodal} fused images from CT, MRI, and PET to show how each can provide different types of information for clinical treatment. \cite{liu2014multimodal} fused data from PET and MRI scans for the diagnosis of Alzheimer's disease.  \cite{subramanian2020multimodal} incorporated imaging data along with genomics data for lung cancer recurrence prediction. Each of these works are similar to ours in the sense that they each are trying to make use of available clinical data. While these methods have shown
improved performance in certain applications, they have disadvantages that stem from their method of  using clinical labels. By using only an additional clinical feature vector associated with already labeled data, these frameworks do not provide a means to incorporate the large pool of unlabeled data into the training process. Our work differs in the sense that by using clinical data alongside a contrastive learning framework we are able to incorporate unlabeled data into the training process, while leveraging the clinical intuition that this information provides. 

\subsection{Deep Learning and OCT}
A desire to reduce diagnosis time and improve timely accurate diagnosis have led to applying deep learning ideas into detecting pathologies and biomarkers directly from OCT slices of the retina. Early work involved a binary classification task between healthy retina scans and scans containing age-related macular degeneration \cite{lee2017deep}. \cite{temel2019relative} introduced a technology to do relative afferent pupillary defect screening through a transfer learning methodology. \cite{kermany2018identifying} showed that transfer learning methods could be utilized to classify OCT scans based on the presence of key biomarkers. \cite{logan2022multimodal} showed how a dual-autoencoder framework with physician attributes could improve classification performance for OCT biomarkers. \cite{prabhushankar2021contrastive} analyzed COVID-19 classification in neural networks to analyze and explain deep learning performance. Subsequent work from \cite{schlegl2018fully} showed that semantic segmentation techniques could identify regions of fluid that are oftentimes indicators of different diseases. \cite{de2018clinically} expanded previous work towards segmentation of a multitude of different biomarkers and connected this with referral for different treatment decisions. \cite{pekala2019deep} showed that segmentation could be done in a fine-grained process by separating individual layers of the retina. Other work has demonstrated the ability to detect clinical information from OCT scans which is significant for suggesting correlations between different domains. \cite{kawczynski2020development} showed that a model trained entirely on OCT scans could learn to predict the associated BCVA value. Similarly \cite{arcadu2019deep} showed that values such as retinal thickness could be learned from retinal fundus photos. All these methods demonstrate the potential for deep learning within the medical imaging domain in the presence of a large corpus of labeled data. On OCT scans where this assumption cannot always be made, contrastive learning methods have grown in popularity. 

\subsection{Contrastive Learning Approaches}
Contrastive learning \cite{le2020contrastive} refers to a family of self-supervised methods that make use of pre-text tasks or embedding enforcement losses with the goal of training a model to learn a rich representation space without the need for labels. The general premise is that the model is taught an embedding space where similar pairs of images project closer together and dissimilar pairs of images are projected apart. Approaches such as \cite{chen2020simple,he2020momentum,caron2020unsupervised, grill2020bootstrap} all generate similar pairs of images through various types of data augmentations such as random cropping, multi-cropping, and different types of blurs and color jitters. A classifier can then be trained on top of these learned representations while requiring fewer labels for satisfactory performance. The authors in~\cite{prabhushankar2021contrastive} augment contrastive class-based gradients and then train a classifier on top of the existing network. Other work \cite{alaudah2019structure, alaudah2018learning} used a contrastive learning setup with a similarity retrieval metric for weak segmentation of seismic structures. \cite{kokilepersaud2022volumetric} used volumetric positions as pseudo-labels for a supervised contrastive loss. Hence, contrastive learning presents a way to utilize a large amount of unlabeled data for performance improvements on a small amount of labeled data. We use this contrastive learning setting on OCT scans. 


Although the aforementioned works have been effective in natural images and other applications, as described in Section~\ref{sec:Intro}, natural image-based augmentations and pretext tasks are insufficient for OCT scans. \cite{rivail2019modeling} introduced a novel pretext task that involved predicting the time interval between OCT scans taken by the same patient. \cite{zhang2021twin} showed how a combination of different pretext tasks such as rotation prediction and jigsaw re-ordering can improve performance on an OCT anomaly detection task. \cite{qiu2019self} showed how assigning pseudo-labels from the output of a classifier can be used to effectively identify labels that might be erroneous. These works all identify ways to use variants of deep learning to detect important biomarkers in OCT scans. However, they differ fundamentally from our work in the sense that they don't present a framework to utilize the abundance of clinical data to aid in the training of a model.

\begin{comment}
Contrastive learning \cite{le2020contrastive} refers to a family of self-supervised methods that make use of pre-text tasks or embedding enforcement losses with the goal of training a model to learn a rich representation space without the need for labels. The general premise is that the model is taught an embedding space where similar pairs of images project closer together and dissimilar pairs of images are projected apart. A classifier can then be trained on top of these learned representations while requiring fewer labels for satisfactory performance. Hence, contrastive learning presents a way to utilize a large amount of unlabeled data for performance improvements on a small amount of labeled data.

Early examples of contrastive learning ideas mostly uilize pre-text tasks where learning of a tangentially related task is utilized specifically for obtaining good representations. This includes work such as \cite{gidaris2018unsupervised} where the authors trained a network to learn features by learning to predict the angle an image has been rotated by. \cite{zhang2016colorful} showed good representations can be learned by predicting colors that should be present given the context in a grayscale image.  \cite{noroozi2016unsupervised} took permutations of tiles extracted within an image and forced the network to learn indices of chosen permutations in a process similar to a jigsaw puzzle. Similar work \cite{doersch2015unsupervised} learned through training to predict the position of patches relative to each other. More modern approaches make use of contrastive losses where low-dimensional embeddings of similar pairs of images are pulled closer together and representations of dissimilar pairs of images are pushed apart. One of the main factors that distinguishes contrastive learning algorithms from each other is how these similar pairs of images are generated or selected. Approaches such as \cite{chen2020simple,he2020momentum,caron2020unsupervised, grill2020bootstrap} all generate similar pairs of images through various types of data augmentations such as random cropping, multi-cropping, and different types of blurs and color jitters. The authors in~\cite{prabhushankar2021contrastive} augment contrastive class based gradients to train a projection head on top of existing networks. These methodologies then utilize various novel frameworks to enforce learning of closeness between the image embedding and the embedding of its augmented version. 
\end{comment}

\subsection{Clinical Labels within Contrastive Learning}
 The literature on self-supervised learning has shown that it is possible to leverage data augmentations as a means to create positive pairs for a contrastive loss. As discussed in the introduction, this isn't so simple within the medical domain due to issues with the diversity of data and small regions corresponding to important biomarkers. Previous work has shown that it is possible to use contrastive learning with augmentations on top of an Imagenet~\cite{deng2009imagenet} pretrained model to improve classification performance for x-ray biomarkers \cite{sowrirajan2020moco}. However, this is sub-optimal in the sense that the model required supervision from a dataset with millions of labeled examples. As a result, recent work has explored the idea of using medically consistent meta-data as a means of finding positive pairs of images alongside augmentations for a contrastive loss function. \cite{azizi2021big} showed that using images from the same medical pathology as well as augmentations for positive image pairs could improve representations beyond standard self-supervision. \cite{chen2021disease} demonstrated utilizing contrastive learning with a transformer can learn embeddings for electronic health records that can correlate with various disease concepts. Similarly, \cite{zhang2020contrastive} utilized pairings of images from x-rays with their textual reports as a means of learning an embedding for classification of various chest x-ray biomarkers. \cite{vu2021medaug} investigated choosing positive pairs from images that exist from the same patient, clinical study, and laterality. \cite{liang2021contrastive} used a contrastive loss to align textual and image embeddings within a chest x-ray setting. \cite{wang2020contrastive} incorporated a contrastive loss to align embeddings from different distributions of CT scans.  These works demonstrate the potential of utilizing clinical data within a contrastive learning framework. However, these methods were tried on limited clinical data settings, such as choosing images from the same patient or position relative to other tissues. Our work builds on these ideas by explicitly using measured clinical labels from an eye-disease setting as its own label for training a model. By doing this, we present a comprehensive assessment of what kinds of clinical data can possibly be used as a means of choosing positive instances from the perspective of OCT scans and expand the scope of how clinical data can be utilized.  This is done by applying novel methods to utilize clinical data in ways that have not been previously explored through creative application of the supervised contrastive loss function. 
 
%%%%%%%%%%%%%%%%%%%%%% Commented out Supervised Contrastive Learning Section and created a more high-level description

 \subsection{Supervised Contrastive Learning}
 The supervised contrastive loss was introduced by \cite{khosla2020supervised} in order to introduce label information within  the traditionally unsupervised contrastive learning framework. The introduced loss function can be represented by: 
 $$
    L_{supcon} = \sum_{i\in{I}} \frac{-1}{|P(i)|}\sum_{p\in{P(i)}}log\frac{exp(z_{i}\cdot z_{p}/\tau)}{\sum_{a\in{A(i)}}exp(z_{i}\cdot z_{a}/\tau)}
$$
 The objective behind this function is to enforce similarity between images with the same label and dissimilarity between images that have differing labels. Using the language of contrastive learning, this means that labels are used to identify the positive and negative pairs, rather than augmentations. The loss is computed on each image $x_{i}$ where $i \in{I}  = {1, ..., 2N}$ represents the index for each instance within the overall augmented batch. Each image $x_{i}$ is passed through an encoder network $f(\cdot)$, producing a lower dimensional representation $r_{i}$. This vector is further compressed through a projection head to produce the embedding vector $z_{i}$. Positive instances for image $x_{i}$ come from the set $P(i)$ and all positive and negative instances come from the set $A(i)$. The loss function operates in the embedding space where the goal is to maximize the cosine similarity between embedding $z_{i}$ and its set of positives $z_{p}$. $\tau$ is a temperature scaling parameter.

 Our work differs from this loss in the sense that we define images belonging to the same class through the use of clinical labels. In this sense, our proposed loss framework can described as a clinically aware supervised contrastive loss. 
 
 %%%%%%%%%%%%%%%%%%%%%% Commented out Supervised Contrastive Learning Section and created a more high-level description
 \begin{comment}
 \subsection{Supervised Contrastive Learning}
 For a set of N random image/label pairs in a random batch $(x_{k},y_{k})_{k=1,...,N}$, the batch is augmented to create a corresponding batch of $2N$ images and labels. This produces a larger set $(x_{l},y_{l})_{l=1,...,2N}$ that consists of two versions of each image that differ only due to random nature of the applied augmentation. Thus for every image $x_{k}$ and label $y_{k}$ there exists two views of the image $x_{2k}$ and $x_{2k-1}$ and two copies of the labels that are equivalent to each other: $y_{2k-1} = y_{2k} = y_{k}$. This set of 2$N$ elements can be considered the multi-viewed batch while the original set of $N$ elements is the starting batch. Within this multi-viewed batch, a loss can be computed on each image $x_{i}$ where $i \in{I}  = {1, ..., 2N}$ represents the index for each instance within the overall batch. For each image an associated embedding vector is generated that is $z_i = \text{Proj}(f(x_{i}))$. The overall loss can be represented as:
$$
    L_{supcon} = \sum_{i\in{I}} \frac{-1}{|P(i)|}\sum_{p\in{P(i)}}log\frac{exp(z_{i}\cdot z_{p}/\tau)}{\sum_{a\in{A(i)}}exp(z_{i}\cdot z_{a}/\tau)}
$$
In this case, the index $i$ represents the specific image within the batch that is acting as the anchor point where embeddings are being pushed or pulled towards. Additionally, $P(i)$ represents the set of all positive instances relative to image $i$ or in other words all instances where $y_{p} = y_{i}$. $|P(i)|$ represents the number of positive instances relative to that specific image in the batch. Finally, $A(i)$ represents all instances in the multi-view batch that constitute the set of negatives and positives for the supervised contrastive loss. In this way, the end result is that we are able to maximize the dot product between embeddings that are positive instances and minimize the dot-product between negative instances in order to complete the objective of the supervised contrastive loss.
\end{comment}



\subsection{OCT Datasets}
Previous OCT datasets for machine learning have labels for specific segmentation and classification tasks regarding various retinal biomarkers and conditions. \cite{kermany2018labeled} contains OCT scans for 4 classes of OCT disease states: Healthy, Drusen, DME, and choroidal neovascularization (CNV). \cite{farsiu2014quantitative} and \cite{melinvsvcak2021annotated} introduced OCT datasets for segmentation of regions with age-related macular degeneration (AMD). \cite{chiu2015kernel} created a dataset for segmentation of regions with DME. In all cases, these datasets do not come with associated comprehensive clinical information nor a wide range of biomarkers to be detected. 
 
Real world clinical studies have the opposing problem where a lot of clinical information is collected, but without explicit biomarker labeling. This is the case with the original source of the data used in this paper: the Prime \cite{hannah2021real} and TREX DME \cite{payne2017randomized,payne2019randomized,payne2021long,wykoff2019intravitreal} experimental trials. Images and clinical information were retrospectively collected at the Retina Consultants of Texas (Houston, TX, USA). Included in this retrospective study were 96 eyes with center-involving diabetic macular edema (CI-DME, n = 56) or diabetic retinopathy without CI-DME (DR, n = 40) between December 2013 and April 2021.

Briefly, both trials were prospective, randomized clinical trials. Prospective trials refer to studies that evaluate the outcome of a particular disease during treatment. In PRIME, 40 eyes with nonproliferative diabetic retinopathy (NPDR) or proliferative diabetic retinopathy (PDR) without CI-DME received intravitreal aflibercept injections (IAI) monthly until the eyes achieved a diabetic retinopathy severity scale (DRSS) score improvement of $\geq$ 2 steps; at baseline, eyes were randomized 1:1 into two management strategies for DR: 1) DRSS-guided or 2) panretinal leakage index (PLI)-guided management. In TREX-DME, 150 eyes with CI-DME were randomized 1:2:2 into three cohorts for management with ranibizumab (0.3 mg): 1) monthly treatment or 2) treat and extend, or 3) treat and extend with angiography-guided macular laser photocoagulation. For each patient, general demographics, ocular disease state data (e.g., best corrected visual acuity (BCVA)), central subfield thickness measurements (CST), and detailed ocular imaging (e.g., spectral-domain optical coherence tomography (SD OCT), fundus photography, and fluorescein angiography) was obtained per the protocol. All SD-OCT images were obtained using the Heidelberg Spectralis HRA+OCT (Heidelberg Engineering, Heidelberg, Germany) with a volume-per-cube acquisition protocol (20 x 20, 49 lines, 768 A-scans per line) with 9-times image averaging. These trials have associated IRB and clinical trial approvals. The IRB approvals are: TREX-DME
IRB: Sterling, 
Protocol: ML28724,
Date of approval: Nov 2013, and
PRIME:
IRB: Quorum,
Protocol: VGFTe-DR-1822,
Date of approval: 5/14/2018. The clinical trial registration numbers are: The Intravitreal Aflibercept as Indicated by Real-Time Objective Imaging to Achieve Diabetic Retinopathy Improvement (PRIME) (ClinicalTrials.gov identifier, NCT03531294)
The Treat and Extend Protocol in Patients with Diabetic Macular Edema (TREX-DME) (ClinicalTrials.gov identifier, NCT01934556)

Our work builds on these clinical studies to add explicit biomarker information to a subset of this data. In this way, we curate a novel dataset that allows experimentation of OCT data from the perspective of both clinical and biomarker labels. 

==> Sections/archive.tex <==
\begin{comment}
\subsection{Combining Biomarkers with Clinical Data}
We also investigate the effect of using a linear combination of losses on a clinical label and biomarker label simultaneously. In this case, we are only able to use the training set of 7500 images present in the Prime + Biomarker dataset. Within this smaller dataset, every image has labels from both the clinical setting as well as the biomarker labels we are interested in detecting. Therefore, in addition to a suspervised contrastive loss with BCVA as the label of interest ($L_{BCVA}$), we can also have a supservised contrastive loss with DME as the label of interest ($L_{DME}$). If we use both of these simultaneously in a combined loss it could look like $L _{total} = L_{BCVA} + L_{DME}$.  In table \ref{tab:supervised_clinical}, each clinical label is used in a supervised contrastive loss with the biomarker we are interested in evaluating performance on. For example, CST + Bio can refer to a supervised contrastive loss of the form:
$$
L _{total} = L_{CST} + L_{DME}
$$
or
$$
L _{total} = L_{CST} + L_{IRF}
$$
The results indicate that incorporating the explicit biomarker label with the clinical label of interest leads to a performance improvement compared to the baseline results of  Table \ref{tab:main_table}. This seems to indicate that the supervised contrastive loss is able to effectively utilize the clinical data for a more fine-grained representation space, while having regularization based on the actual biomarker label of interest. 

\begin{table}[]
\centering
\begin{tabular}{@{}cccc@{}} 

\toprule
\multicolumn{3}{c}{Biomarker + Clinical (Accuracy / F1-Score)}                       \\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{IRF} & 
\multicolumn{1}{c|}{DME} \\ \midrule
Supervised                &   &  \\
Fusion Supervised                 &  &  \\
PCL                & 76.50\% / .717  & 80.11\% / .761 \\
SimCLR                 & 75.13\% / .715 & 80.61\% / .772 \\
Moco v2                 & 76.00\% / .720    &  82.84\% / .793 \\ \bottomrule
Eye ID + Bio                & \textbf{77.93}\% / .742  & 83.36\% /.807  &  \\
CST + Bio               & 77.46\% / .727  & \textbf{83.57}\% / \textbf{.809}  \\
BCVA + Bio                 & 77.8\% / .741  & 81.7\% / .790  \\
BCVA + Eye ID + Bio               &  74.13 \% / .691 & 80\% /  .762    \\
BCVA + CST + Bio                 & 76.3\% / .710  & 81.53\% / .782   \\
CST + Eye ID + Bio               & 77.83\% / \textbf{.747}& 82.93\% / .804 \\
BCVA + CST + Eye ID  + Bio              & 75.06\% /.705  & 80.816\% /.772  \\


 \bottomrule
\end{tabular}
\caption{Supervised Contrastive Learning on using the biomarker label in tandem with the clinical label for IRF and DME.}
\label{tab:supervised_clinical}
\end{table}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Commented out the Alpha Parameter Tuning
\subsection{Alpha Parameter Tuning}
In this section, the impact of adding an alpha parameter to effectively weight the contribution of the loss from each individual clinical value is evaluated. From the results in Table \ref{tab:alpha_tuning} it is inconclusive as to whether weighting this loss actually has a positive impact on performance. In the case of $\alpha$ BCVA + (1-$\alpha$) Eye ID and $\alpha$ CST + (1-$\alpha$) Eye ID performance in terms of the multilabel AUROC metric actually decreased. This may indicate that in these combined clinical loss functions, neither clinical label is inherently more informative than the other. It may be the case that each is able to contribute through it's own respective positive pairs to the overall loss and weighting one against the other doesn't allow this advantage to be utilized.
\begin{table}[]
\centering
\begin{tabular}{@{}cccccc@{}}

\toprule
\multicolumn{6}{c}{Alpha Tuning Experiments}                  \\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{Original} &
\multicolumn{1}{c|}{$\alpha$ = .2} & 
\multicolumn{1}{c|}{$\alpha$ = .4} &   




\multicolumn{1}{c|}{$\alpha$ = .6} &
\multicolumn{1}{c|}{$\alpha$ = .8}\\ \midrule
$\alpha$BCVA + (1-$\alpha$)CST & .7875 & .7782 & .7871 & .7901 & .7898 \\
$\alpha$BCVA + (1-$\alpha$)Eye ID              & .806  & .7928 & .7902 & .7925 & .7945 \\
$\alpha$CST + (1-$\alpha$)Eye ID                    & .801  & .7795 & .7898 & .787 & .7841 \\



 \bottomrule
\end{tabular}
\caption{Experiment on varying the weighting between losses derived from using each clinical value as a label. Performance is measured with an average AUROC score metric.}
\label{tab:alpha_tuning}
\end{table}
\end{comment}


==> Sections/experiments_no_highlights.tex <==


\subsection{Training Details}
Care was taken to ensure that all aspects of the experiments remained the same whether training was done via supervised or self-supervised contrastive learning on the encoder or cross-entropy training on the attached linear classifier. The encoder utilized was kept as a ResNet-50 architecture. The applied augmentations are random resize crop to a size of 224, random horizontal flips, random color jitter, and data normalization to the mean and standard deviation of the respective dataset. The batch size was set at 128. Training was performed for 25 epochs in every setting. A stochastic gradient descent optimizer was used for contrastive pre-training with a learning rate of .05, weight decay of .0001, and momentum of .9. The same chosen hyper-parameters were used during cross-entropy fine-tuning except the learning rate was changed to .001 for stability during this step. The comparison methods of SimCLR\cite{chen2020simple}, Moco v2\cite{chen2020improved}, and PCL \cite{li2020prototypical} were trained in the same manner with certain hyper-parameters specific to each method. Specifically, Moco v2 was set to its default queue size of 65536. Additionally, PCL has hyper-parameters specific to its clustering step, but the original documentation made these parameters specific to the Imagenet \cite{deng2009imagenet} dataset on which it was originally built for. To fit these parameters to our setting, the clustering step was reduced in size.

\subsubsection{Metrics and Notation}
During supervised contrastive training, a choice of a single clinical parameter or combination of parameters is chosen to act as labels. For example, in Table \ref{tab:individual_biomarker_table} when the method is specified as BCVA this indicates a supervised contrastive loss $L_{BCVA}$ where BCVA is utilized as the label of interest for the images in the dataset. Additionally, BCVA + CST refers to a linear combination of supervised contrastive losses that can be expressed as $L_{BCVA+CST} = L_{BCVA} + L_{CST}$ where each clinical value respectively  acts as a label for its respective loss. A linear layer is then appended to this trained encoder and trained on the biomarker labels present, which consists of approximately 7,500 images during training. This linear layer is trained on each biomarker individually and accuracy as well as F1-score in detecting the presence of each individual biomarker is reported. Any table that reports the standard average area under the receiver operating curve (AUROC) is reporting the AUROC calculated after finding the AUROC for each individual biomarker test set and then averaging them together in order to get a single metric summarizing performance. The same is done to get an average precision, sensitivity, and specificity. Performance is also evaluated in a multi-label classification setting where the goal is to correctly identify the presence or absence of all 5 biomarkers at the same time. This is evaluated using averaged AUROC over all 5 classes within this multi-label setting. Every reported value is the average of 3 runs of the specified method and the standard deviation for both accuracy and AUROC are reported.
\begin{figure}[t]
\centering
\includegraphics[scale = .4]{images/tsne_plot.jpg}
\caption{Images from the OLIVES Biomarker dataset labeled by the presence or absence of DME and Fluid IRF were fed into an encoder network trained by using BCVA values as the label as well as a SimCLR strategy. This produced an embedding for each image. These embeddings were visualized using t-SNE \cite{van2008visualizing}  with two components. It can be observed that from an encoder trained using BCVA labels with the supervised contrastive loss, we can effectively achieve an embedding space that is separable with respect to biomarkers while the standard contrastive learning method shows no separability for either of the biomarkers. }
\label{fig: dme_ebed}
\end{figure}


%%%%%%%%% Table shows average AUROC across all biomarkers across different splits of patients
\begin{table}[]
\centering
\scalebox{.8}{
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{5}{c}{Averaged AUROC Across Different Splits Of Patients}   
\\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{PS1} & \multicolumn{1}{c|}{PS2} & \multicolumn{1}{c|}{PS3} & \multicolumn{1}{c|}{Average}\\\midrule
PCL  \cite{li2020prototypical}  &   $.676 \pm .002$ & $.759 \pm .002$ & $.779 \pm .002$ & $.738 \pm .054$            \\

SimCLR \cite{chen2020simple}     &   $.761 \pm .003$ & $.770 \pm .001$ & $.795 \pm .001$ & $.775 \pm .018$               \\
Moco v2 \cite{chen2020improved}  &   $.737 \pm .002$ & $.769 \pm .002$ & $.729 \pm .002$ & $.745 \pm .021$           \\ \bottomrule

Eye ID   &   $.802 \pm .001$ & $.782 \pm .001$ & $ .801 \pm .001$ & $.795 \pm .006$                 \\ \hline
CST     &   $.793 \pm .001$ & $.794 \pm .001$ & $.783 \pm .001$ & $.790 \pm .006$                   \\
BCVA    &   $.801 \pm .001$ & $.788 \pm .001$ & $.776 \pm .001$ & $.788 \pm .012$                \\

BCVA + Eye ID  &   $.804 \pm .002$ & $.796 \pm .001$ & $.821 \pm .001$ & $.807 \pm .013$          \\

BCVA + CST  &   $.807 \pm .001$ & $.795 \pm .001$ & $.797 \pm .001$ & $.800 \pm .007$             \\
CST + Eye ID  &   $\textbf{.819} \pm .001$ & $\textbf{.833} \pm .001$ & $\textbf{.828} \pm .001$ & $\textbf{.827} \pm .007$        \\

BCVA + CST + Eye ID  &   $.817 \pm .001$ & $.792 \pm .001$ & $.821 \pm .001$ & $.810 \pm .015$        \\

 \bottomrule
\end{tabular}}
\caption{We show performance in terms of average AUROC across all biomarkers for different training and testing splits for patient groups. PS1, PS2, and PS3 refer to the three different patient splits created. The average column refers to the average performance across all the splits. We also performed a statistical significance test over the resultant average performance. A green highlight indicates that the result is significant with respect to the best result on all patient splits and red indicates that the result lacked statistical significance. The threshold used to determine significance is a p-value of .05. }
\label{tab:patient_split_table}
\end{table}

%%%%%%%%% Table shows average AUROC for other clinical parameters
\begin{table}[]
\centering
\begin{tabular}{@{}cc@{}}
\toprule
\multicolumn{2}{c}{Averaged AUROC on Smaller Contrastive Subset}   
\\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{AUROC} \\\midrule
PCL  \cite{li2020prototypical}     & $.667 \pm .006$         \\

SimCLR \cite{chen2020simple}       & $.689 \pm .002$             \\
Moco v2 \cite{chen2020improved}    & $.559 \pm .002$              \\ \bottomrule

Eye ID        & $.748 \pm .001$             \\ \hline
CST          & $.781 \pm .001$               \\
BCVA               & $.775 \pm .002$          \\

Leakage Index        & $\textbf{.801} \pm .001$      \\

DRSS        & $.618 \pm .002$         \\
Diabetes Type    & $.646 \pm .007$          \\

Years with Diabetes  & $.761 \pm .001$      \\
Gender  & $.609 \pm .003$      \\

 \bottomrule
\end{tabular}
\caption{To study the impact of reducing the amount of available training data during the contrastive training set, we utilized the PRIME subset of the OLIVES dataset for training the ResNet-50 network. In this case, we have access to additional clinical values that we can observe because this subset has additional clinical information that can be investigated. We use the average AUROC across all biomarkers as the metric of interest.}
\label{tab:clinical_diverse_table}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Figure of ResNet-18 vs ResNet-50 performance
%%%%%%%%% Table shows average AUROC for other clinical parameters
\begin{table}[]
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
\multicolumn{3}{c}{Averaged AUROC on Different Sized Architectures}   
\\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{R-18} & \multicolumn{1}{c|}{R-50} \\\midrule
PCL  \cite{li2020prototypical}     & $.716 \pm .002$ & $.676 \pm .002$         \\

SimCLR \cite{chen2020simple}      & $.719 \pm .002$ & $.761 \pm .003$              \\
Moco v2 \cite{chen2020improved}    & $.748 \pm .002$ & $.737 \pm .002$              \\ \bottomrule

Eye ID        & $.771 \pm .001$ & $.802 \pm .001$             \\ \hline
CST          & $.771 \pm .003$ & $.793 \pm .001$               \\
BCVA          & $.753 \pm .002$ & $.801 \pm .001$               \\

BCVA + Eye ID    & $.792 \pm .003$ & $.804 \pm .002$          \\

BCVA + CST      & $.796 \pm .002$ & $.807 \pm .001$           \\
CST + Eye ID   & $.794 \pm .004$ & $\textbf{.819} \pm .001$          \\

BCVA + CST + Eye ID  & $ \textbf{.816} \pm .004$ & $.817 \pm .001$      \\

 \bottomrule
\end{tabular}
\caption{This table shows the average AUROC metric across all biomarkers for different sized architectures. R-18 and R-50 refers to ResNet-18 and ResNet-50 \cite{he2016deep} respectively.}
\label{tab:arch}
\end{table}
\subsection{Biomarker Detection Experiments}
We first evaluate the capability of our method to leverage a larger amount of clinical labels for performance improvements on the smaller biomarker subset. This involves supervised contrastive training of the encoder network on the training set with clinical labels, consisting of approximately 60,000 images. Tables \ref{tab:individual_biomarker_table} and \ref{tab:all_biomarker_table} shows that applying our method of choosing positives and negatives based on some clinical label or combination of labels leads to improvements on classification accuracy and f1-score of each biomarker individually as well as an improved average AUROC, precision, sensitivity, and specificity over all 5 biomarkers when compared against state of the art self-supervised algorithms. We can also observe visually how well training on a clinical label performs in creating a separable embedding space for biomarkers through Figure \ref{fig: dme_ebed}. This figure was generated by taking a model trained with a supervised contrastive loss on BCVA values as well as a model trained with the SimCLR framework and inputting the test set labeled by the biomarkers DME and Intraretinal Fluid. This produces embeddings for each image in the test set. These embeddings are projected into a lower dimensional space with 2-D t-SNE \cite{van2008visualizing} algorithm. It can be observed that the resulting representation can separate between present and absent forms of DME and Fluid IRF without having explicit training for these labels. However, the model trained with just self-supervision shows almost no separability with respect to these biomarkers. This acts as validation to the relationship between both the clinical labels and biomarkers and gives insight into the improved results that we observe.  

Other interesting conclusions can be derived from observing the performance of the standard self-supervised methods compared to our clinically driven concepts. It is  observed in Table \ref{tab:individual_biomarker_table} that the self-supervised algorithms are comparable to our methods for IRF and DME, but are worse for IRHRF, FAVF, and PAVF. In other words, the traditional contrastive learning algorithms did comparably well on biomarkers that were easy to distinguish from the rest of the image, but did poorly on biomarkers that exhibited a higher degree of granularity.
This difference can be understood through the analysis performed by the authors of \cite{cole2021does}. In this work, the authors showed that the performance gap between contrastive learning and supervised learning increases as the granularity of the task correspondingly increases. They hypothesized that the contrastive loss tends to cluster images based on coarse-visual similarity. This is because the contrastive loss relies on creating positive instances of similar images from augmentations taken from an individual image. In this sense, there is a dependence on the individual image itself to have enough distinguishable features such that a contrast can be created with the negative instances in the loss function. This may not always be the case, especially when it comes to the medical domain where images can be very similar with the exception of small localized regions. We hypothesize that our method is better able to overcome this issue by providing an effective method to identify positive instances that are correlated through having similar clinical metrics. Instead of an over-reliance on augmentations from a single image, a more robust set of positive pairs can be found that allows the model to more effectively identify fine-grained features of OCT scans.  This is due to having a wider and more informative set of features to treat as positive instances, thus allowing the model to better identify distinguishing features when using a contrastive loss even for more fine-grained cases. 

Another aspect of the results in Table \ref{tab:individual_biomarker_table} is how well the used clinical labels correspond with the biomarker classification performance. In all cases, the results act as validation to the hypothesis that taking advantage of correlations that exist with certain clinical labels is beneficial for biomarker detection of individual OCT scans. However, from a medical perspective, certain outcomes would intuitively be more likely. For example, for IRF and DME it makes sense that the best performance is associated with using CST values because CST tends to more closely increase or decrease, depending on the severity of IRF and DME. In general, further medical insight is needed to determine what is expected in terms of the degree of correlations between biomarkers and individual clincal values. 


\subsection{Robustness Experiments}

In this section, we investigate the performance of our algorithms in a variety of settings meant to test how robust our method is to various perturbations in the original setup. This includes different training and test splits based on different subsets of the patient pool, experiments where we reduce the amount of clinical and biomarker training data, studies on different sized backbone architectures, and experiments within the tougher setting of multi-label classification. In all experiments we summarize performance as the average of the AUROC found on each biomarker test set. Through these experiments we arrive at the somewhat surprising finding that using a combination of clinical labels in a linear combination of supervised contrastive losses actually out-performs all other methods whether self-supervised or on individual clinical labels. 

In our first experiment, we create two new training and test sets based on splitting by patient identities. We show in Table \ref{tab:patient_split_table} that our methods work even in the case where splits between training and testing are made on the basis of different patient identities than the one we originally started with. When we take the average across all patient identity splits, it should be noted that methods that utilized a combined loss such as CST + Eye ID were able to maintain a consistently higher performance across different splits, while maintaining a much lower variance across splits. This difference is further highlighted when comparing against the self-supervised algorithms which exhibited not only lower performance, but also a greater variance across the different splits. All of this indicates that these combined losses have a greater robustness with respect to whichever training and testing pool is utilized. A possible reason for this is that each clinical value can be thought of being associated with its own distribution of images. By having a linear combination of losses on two clinical values, we are effectively choosing positive instances from closely related, but slightly varying distributions. These distributions are visualized in Figures \ref{fig:bcva_dist} and \ref{fig:cst_dist}. It can be observed that because BCVA and CST have different ranges of potential values, as observed along the x-axis of this figure, this means that for any individual value there is a different number of associated eyes and images. Effectively, this means that there is varying diversity with respect to any individual label. This may allow the model to better learn features by allowing the model to sample from different proposal distributions that may better approximate the true disease severity distribution. 

We also observe the robustness of the combined clinical losses in the setting of different architecture choices. We see in Table \ref{tab:arch} that the combined clinical losses were the only ones that maintained consistently high performance across both the ResNet-18 and ResNet-50 architectures. Additionally, we see that in the case of self-supervised methods, PCL and SimCLR actually did worse on the larger architecture. This may be due to over-fitting on the easily distinguishable features while losing the ability to generalize to the higher granularity biomarkers. 

From a medical perspective, the success of our approach across patient, architecture, and eye splits is indicative of its generalizability. Fully self-supervised approaches are dependent on the data to have enough differentiating features such that augmentations can be used to learn useful features. In this sense, certain groups of patients will potentially be more informative than others, which limits the ability of these approaches to generalize. However, our approach, by choosing positives from a much wider set of data, does not have as strong of a dependence on the features present in any one image. From this perspecitve, there is a greater robustness in regards to patient distributions which corresponds to the better performance across all splits of data.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Potential Table of Multi-Label Classification Performance
\begin{comment}
\begin{table}[]
\centering
\begin{tabular}{@{}cc@{}}
\toprule
\multicolumn{2}{c}{Averaged AUROC in Multi-Label Classification Setting}   
\\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{AUROC} \\\midrule
PCL  \cite{li2020prototypical}  & $.681 \pm .002$            \\

SimCLR \cite{chen2020simple}  & $.727 \pm .002$                  \\
Moco v2 \cite{chen2020improved}  & $.734 \pm .002$                \\ \bottomrule

Eye ID      & $.795 \pm .001$               \\
CST         & $.749 \pm .003$                \\
BCVA        & $.790 \pm .002$                 \\

BCVA + Eye ID  & $.795 \pm .002$            \\

BCVA + CST     & $.782 \pm .001$            \\
CST + Eye ID   & $ \textbf{.806} \pm .003$          \\

BCVA + CST + Eye ID & $.806 \pm .002$       \\

 \bottomrule
\end{tabular}
\caption{This shows the performance of the average AUORC metric across all biomarkers in a multi-label classifications setting where the model is tasked with detecting all present biomarkers at once.}
\label{tab:multi-label}
\end{table}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Potential Figure of Different Amounts of Biomarker Accesss

\begin{table}[]
\centering
\scalebox{.8}{
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{5}{c}{Averaged Multi-Label AUROC with varying Biomarker Access}   
\\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{25\%} & \multicolumn{1}{c|}{50\%} & \multicolumn{1}{c|}{75\%} & \multicolumn{1}{c|}{100\%}\\\midrule
Supervised & $.703 \pm .002$ & $.716 \pm .003$ & $.719 \pm .002$ & $.722 \pm .005$ \\

PCL  \cite{li2020prototypical}  &   $.675 \pm .003$ & $.681 \pm .004$ & $.683 \pm .002$ & $.681 \pm .002$            \\

SimCLR \cite{chen2020simple}     &   $.679 \pm .004$ & $.709 \pm .006$ & $.718 \pm .003$ & $.727 \pm .002$               \\
Moco v2 \cite{chen2020improved}  &   $.709 \pm .006$ & $.722 \pm .002$ & $.732 \pm .001$ & $.734 \pm .002$                \\ \bottomrule

Eye ID   &   $.754 \pm .005$ & $.778 \pm .003$ & $.789 \pm .001$ & $.795 \pm .001$                  \\ \hline
CST     &   $.694 \pm .004$ & $.721 \pm .003$ & $.739 \pm .001$ & $.749 \pm .001$                    \\
BCVA    &   $.760 \pm .009$ & $.788 \pm .001$ & $.783 \pm .001$ & $.790 \pm .001$                \\

BCVA + Eye ID  &   $.761 \pm .004$ & $.786 \pm .004$ & $.794 \pm .002$ & $.795 \pm .002$            \\

BCVA + CST  &   $.712 \pm .005$ & $.751 \pm .007$ & $.773 \pm .006$ & $.782 \pm .001$               \\
CST + Eye ID  &   $\textbf{.766} \pm .013$ & $\textbf{.786} \pm .003$ & $\textbf{.803} \pm .004$ & $\textbf{.806} \pm .003$             \\

BCVA + CST + Eye ID  &   $.747 \pm .005$ & $.778 \pm .003$ & $.802 \pm .004$ & $.806 \pm .002$        \\

 \bottomrule
\end{tabular}}
\caption{This table shows the average AUORC in a multi-label classification with different amounts of access to biomarker data for fine-tuning the model.}
\label{tab:biomarker_split_table}
\end{table}

Throughout the paper so far, all experiments have been done on a dataset that was based on the total \texttt{OLIVES} dataset that is derived from two clinical trials. However, in order to study the impact of reducing the amount of avilable data for contrastive pre-training, we extract the clinical labels and image from just the PRIME \cite{hannah2021real} clinical trial. this reduces the overal contrastive training pool to 29000 images. There are several interesting analytical points that we can draw from doing this. The first is that the PRIME subset has a wider variety of clinical information that we can potentailly use as a label. In addition to BCVA, CST, and Eye ID that are available across the whole \texttt{OLIVES} dataset; there are clinical parameters that exist for the PRIME subset specifically such as the type of diabetes of the patient, the diabetic retinopathy severity score (DRSS), and various demographic information. It can be observed that while CST, BCVA, and Eye ID still perform consistently well, there are other modalities that perform better than the self-supervised baselines. This includes leakage index and the number of years with diabetes. This indicates that there are potentially many unexplored clinical values in a variety of settings that have the potential to choose good positives and negatives for a contrastive loss. A possible reason for the huge difference in performance between the clinical and self-supervised methods is that Prime alone has fewer images as well as less image diversity compared to the total OLIVES dataset. As a result, regular self-supervised methods are more constrained in the representations that can be drawn from just taking augmentations to form positive pairs in a contrastive loss. In this way, they are more dependent on the total number of images in the training set as well as the total available data diversity.

We also analyze the impact of training with a progressively limited set of biomarker data.  To do this, we take our original training set of 7500 labeled biomarker scans and remove different sized subsets. This is shown in Table \ref{tab:biomarker_split_table} where each column represents the percentage amount of biomarker training data we restricted each method to have access to. We observe that using our contrastive learning strategy leads to improved performance in the multi-label classification setting. Additionally, strategies that make use of a combined clinical loss  again more consistently have a high performance even with reduced access to data for biomarker fine-tuning. Furthermore, for this table, we include a comparison with a network trained from scratch on the biomarker data only, using the same hyper-parameters as all previous experiments. This acts as an analysis of a semi-supervised setting since labeled data is progressively removed. It is interesting to note that the supervised methods, that have access to the biomarker labels during the entirety of training, are significantly worse as the training set is reduced. This shows the dependence that these methods have on a large enough training set because they are unable to leverage representations that may be learnt from the large unlabeled pool of data. The self-supervised methods we compare against are better able to make use of these representations to perform better on the smaller amount of available training data, but are still inferior to our method that integrates clinical labels into the contrastive learning process. An additional reason for this difference is the difficulty of the multi-label classification task. Within this task, certain biomarkers are easier to learn than others and it is possible that without sufficient training data these models more readily learn the features of the easier to detect classes and neglect the classes that exist as higher granular features. 

\begin{table}[]
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
\multicolumn{3}{c}{Semi-Supervised Setting Performance (Accuracy/F1-Score)} \\ \midrule
                  & SimCLR v2 \cite{chen2020big}                 & CST + Eye ID               \\ \midrule
DME               & 68.66\% / .594             & \textbf{71.13}\% / \textbf{.696}             \\
IRF               & 63.73\% / .586             & \textbf{65.73}\% / \textbf{.590}             \\
IRHRF             & 57.13\% / .350             & \textbf{57.8}\% / \textbf{.553}              \\
FAVF              & 52.80\% / .503             & \textbf{54.30}\% / \textbf{.643}             \\
PAVF              & 47.60\% / \textbf{.183}             & \textbf{48.20}\% / .166             \\ \bottomrule
\end{tabular}
\caption{This table analyzes the integration of a clinical contrastive method into a state of the art semi-supervised framework \cite{chen2020big}.}
\label{tab:semi}
\end{table}

\subsection{Comparison with Eye Identity}
In \cite{vu2021medaug,diamant2021patient,azizi2021big}, the authors created a contrastive learning strategy based on choosing positives and negatives based on the patient identity. In order to create a comparison with these previously proposed approaches, we designate the strategy that chooses positives and negatives based on just the eye identity as its own separate section within each table that reflects the suggestion of these previous works. It can be observed that this method does perform better than the self-supervised baselines, as pointed out in previous work, but it does not do as well as our methods that make use of multiple clinical distributions such as CST + Eye ID. In Table \ref{tab:individual_biomarker_table}, methods that use other types of clinical labels or multiple clinical labels in tandem out-perform Eye ID on 4 out of the 5 biomarkers in terms of accuracy and f1-score. The same trend holds when looking at the patient split experiments in Table \ref{tab:patient_split_table}. Additionally, Eye ID consistently performs worse than methods that make use of multiple clinical distributions within the other robustness experiments that vary access to biomarker and clinical training data in Tables \ref{tab:biomarker_split_table} and \ref{tab:clinical_diverse_table}. This indicates that while patient/eye identity is an improvement over standard self-supervision, other individual clinical labels and their combinations can potentially offer better distributions on which positives and negatives for a contrastive loss can be sampled. 


\subsection{Semi-Supervised Experiments}
We also compare our method within a state of the art semi-supervised framework in Table \ref{tab:semi}. In this case, we follow the setting of \cite{chen2020big}. To do this we take an encoder pre-trained with a contrastive learning strategy and fine-tune it with a linear layer with only 25\% of available biomarker data for each biomarker in this study. This model then becomes the teacher model that we use to train a corresponding student model. The student model has access to both the 25\% subset the teacher was trained on as well as the remaining biomarker data that we designate to be the unlabeled subset. The teacher is used to provide logit outputs that is then used as part of a distillation loss discussed in \cite{chen2020big} to train the student model. In this way, we model the semi-supervision setting by making use of a small amount of labeled data for the teacher model and then both labeled and unlabeled data for the student. We compare the performance of this setup on a pretraining with respect to SimCLR and our combined clinical contrastive strategy that makes use of both the CST and Eye ID label distributions. We observe in Table \ref{tab:semi}  that our method consistenly out-performs the model that used SimCLR pre-training. It is also interesting to note that the overall performance is lower than in the standard contrastive learning setting. Part of the reason for this is that this setup assumed access to a large unlabeled pool on the order of the size of ImageNet \cite{deng2009imagenet}. In this case, the teacher network may not have enough labels to initially fine-tune with and the corresponding distillation loss for the student network does not have enough unlabeled data to effectively impute the knowledge onto the student network. Despite the limitations of this constrained setting, we still see that our method is able to out-perform the SimCLR v2 baseline.

\subsection{Limitations}
While our analysis provides an in-depth look into the relationship between clinical and biomarker data for contrastive learning, there are still areas where further exploration is difficult to perform due to constraints of the medical setting. Specifically, part of the novelty of our analysis is derived from demonstrating the performance degradation of biomarkers as we approach higher levels of granularity. This shows that the conclusions of \cite{cole2021does} do have the potential to transfer within a medical setting. However, due to the difficulty of access to a sufficient amount of biomarker data we cannot perform an all-encompassing experiment of this granularity concept within a medical setting. Additionally, it is difficult to quantify this concept of granularity. We can intuitively get a sense of which biomarkers exhibit high and low granularity from medical studies such as \cite{markan2020novel}, but it remains somewhat hypothetical as to exact meaning of granularity. Furthermore, ideally this entire setting could be studied in many other contexts, but in most cases access to well-distributed clinical data as well as biomarkers is difficult to find in publicly available datasets which highlights the importance of the \texttt{OLIVES} dataset for this study. We encourage medical and machine learning practitioners to use the ideas presented in this paper as inspiration for the proper usage of clinical data within their own application settings.  

==> Sections/methodology_no_highlights.tex <==



\subsection{Dataset}

\begin{figure*}[ht]
\centering
\includegraphics[scale = .4]{images/methodology.jpg}
\caption{ Overview of Experimental Setup. 1) Supervised contrastive learning is performed on the larger amount of available clinical data provided in OLIVES Clinical. 2) This trained encoder then has its weights frozen and a linear classifier is trained utilizing the smaller amount of data from the OLIVES Biomarker dataset.}
\label{fig: supcon}
\end{figure*}
 We make use of the \texttt{OLIVES} \cite{prabhushankar2022olives} dataset for our studies. This dataset is composed of 78108 OCT scans from two clinical trials. Every image is associated withe the clinical information of Eye identity, BCVA, and CST that was naturally collected during the process of patient treatment during the clinical trial. A smaller subset of 9408 images was additionally labeled by a trained grader for the presence or absence of 16 different biomarkers present in each image.   In addition to this information provided by the studies, a trained grader performed interpretation on OCT scans for the presence of 20 different biomarkers including: Intra-Retinal Hyper-Reflective Foci (IRHRF), Partially Attached Vitreous Face (PAVF), Fully Attached Vitreous Face (FAVF), Intra-Retinal Fluid (IRF), and Diffuse Retinal Thickening or Macular Edema (DRT/ME). The trained grader was blinded to clinical information whilst grading each of 49 horizontal SD-OCT B-scans of both the first and last study visit for each individual eye. This results in a subset of both studies now having just clinical labels and a smaller subset having both clincial and biomarker labels as observed in Figure \ref{fig:quantity}. This can be further understood by Figure \ref{fig: image_single_example} where we can see that, for a single image, a wide variety of both clinical and biomarker labels can exist.  Open adjudication was done with an experienced retina specialist for difficult cases.


As a result, for each OCT scan labeled for biomarkers, there exists a one-hot vector indicating the presence or absence of 16 different biomarkers. Not all of these 16 biomarkers exist in sufficiently balanced quantities to train a model to identify their presence or absence within an image. Hence, we use Intraretinal Hyperreflective Foci (IRHRF), Partially Attached Vitreous Face (PAVF), Fully Attached Vitreous Face (FAVF), Intraretinal Fluid (IRF), and Diffuse Retinal Thickening or Diabetic Macular Edema (DRT/ME) as the biomarkers that are studied in this paper. These biomarkers were also chosen in order to enable a novel granularity analysis as discussed in the introduction. From Figure \ref{fig: examples} we observe that the biomarkers of IRF and DME exhibit low granularity in the sense that they are easily distinguishable, while the biomarkers IRHRF, PAVF, and FAVF are features with high granularity that are hard to rectify from the rest of the image.  It should be noted that because OLIVES dataset is composed of images from two separate trials with different intended outcomes, this results in each having different types of clinical information. When combining the trials together, we only focus on the clinical data that is commonly held by both trials: BCVA, CST, and Eye ID.  We present the manifestation of distributions within the OLIVES dataset for the clinical values of BCVA, CST, and Eye ID in Figures \ref{fig:patient_dist}, \ref{fig:bcva_dist}, and \ref{fig:cst_dist}. It can be observed that the distribution of each value image quantities isn't noticeably biased towards any specific value. Instead, for each value, there is diversity in terms of the number of different eyes and number of images. 


In total, the \texttt{OLIVES} dataset provides data from 96 unique eyes and 87 unique patients. We take 10 unique eyes from both clinical trials in the \texttt{OLIVES} dataset and use the data from these 20 eyes to create the test set. The remaining 76 eyes are utilized for training in all experiments. Since the objective is to evaluate the model's performance in identifying each biomarker individually, a test set for each biomarker is created. This is done by randomly sampling 500 images with the biomarker present and 500 images with the biomarker absent from the data associated with the test eyes. In this way, we ensure that the test set for each individual biomarker is balanced.

In the case of nine patients there exists data for the left and right eye. This leads to questions as to whether this may potentially bias any experiments that are performed by having both in the dataset. However, in the original clinical trials on which \texttt{OLIVES} is based, each eye is treated as independent from every other eye and different experimental settings are applied to each. Consequently, random splits of experiments were made on the basis of the eye identity, rather than the patient identity. This also means that data is recorded for individual eyes, rather than individual patients. So as to align with the setup of the original studies, we make our train and test split on the basis of the eye identity. Ablation studies later in the paper show that our methods perform comparably even if we were to make the split based solely on patient identity.


\begin{table*}[]
\centering
\begin{tabular}{@{}cccccc@{}}
\toprule
\multicolumn{6}{c}{Individual Biomarker Performance (Accuracy / F1-Score)}   
\\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{IRF} & \multicolumn{1}{c|}{DME} & \multicolumn{1}{c|}{IRHRF} & \multicolumn{1}{c|}{FAVF} & \multicolumn{1}{c|}{PAVF} \\\midrule
PCL  \cite{li2020prototypical} &  $74.45\% \pm.212 / .687$ & $78.74\% \pm.510 / .741$ & $56.36\% \pm.404 / .663$ &  $53.43\% \pm.057 / .635$ & $50.06\% \pm.305 / .028$             \\

SimCLR \cite{chen2020simple}  &  $74.16\% \pm.115 / .689$ & $79.44\% \pm.154 / .758$ & $61.53\% \pm1.19 / .679$ &  $73.53\% \pm.305 / .739$ & $53.90\% \pm.519 / .269$                  \\
Moco v2 \cite{chen2020improved} &  $\textbf{76.23}\% \pm.208 / .721$ & $77.89\% \pm.101 / .724$ & $57.20\% \pm.360 / .678$ &  $64.70\% \pm.458 / .696$ & $51.80\% \pm.400 / .119$               \\ \bottomrule

Eye ID  &  $73.20\% \pm.100 / .692$ &$77.58\% \pm.268 / .740$ & $58.90\% \pm.529 / .681$ &  $82.00\% \pm.100 / .841$ & $\textbf{68.53}\% \pm.208 / \textbf{.604}$                \\
\hline
CST   &  $73.83\% \pm.057 / .670$ & $78.66\% \pm.058 / .736$ & $61.33\% \pm.057 / .676$ &  $79.23\% \pm.351 / .797$ & $57.96\% \pm.152 / .372$                 \\

BCVA  &  $74.13\% \pm.152 / .689$ & $80.32\% \pm.101 / .766$ & $\textbf{63.83}\% \pm.321 / \textbf{.692}$ &  $78.90\% \pm.529 / .800$ & $60.93\% \pm.208 / .452$   \\

BCVA + Eye ID &  $73.30\% \pm.435 / .701$ & $80.02\% \pm.101 / .775$ & $55.93\% \pm.473 / .679$ &  $\textbf{82.56}\% \pm.305 / \textbf{.843}$ & $66.16\% \pm.115 / .561$             \\

BCVA + CST  &  $74.26\% \pm.208 / .695$ & $80.22\% \pm.101 / .765$ & $62.00\% \pm.400 / .681$ &  $81.00\% \pm.100 / .818$ & $60.66\% \pm.416 / .447$   \\              
CST + Eye ID  &  $75.66\% \pm.152 / \textbf{.728}$ & $\textbf{80.86}\% \pm.154 / \textbf{.786}$ & $59.13\% \pm.208 / .686$ &  $80.60\% \pm.200 / .825$ & $60.53\% \pm.551 / .436$            \\

BCVA + CST + Eye ID  &  $74.26\% \pm.416 / .697$ & $80.15\% \pm.058 / .765$ & $61.43\% \pm.305 / .692$ &  $82.33\% \pm.057 / .837$ & $62.16\% \pm.057 / .492$        \\

 \bottomrule
\end{tabular}
\caption{This table shows the performance of each contrastive training strategy in terms of accuracy and F1-Score for each individual biomarker used in this study. We also perform a significance test for the best result associated with each biomarker. This was done by running 3 different trials for every method on different seeds to produce a population of model outputs associated with each method. We then perform a pairwise t-test between the population of outputs for the best performing model and every other model in the column to compare whether the means of the output performance for the two groups are significantly different from each other. If the p-value generated by this test was less than .05 we deemed the performance difference between the best model and the tested model as significant and highlighted it as green in the table above.}
\label{tab:individual_biomarker_table}
\end{table*}
\subsection{Overall Framework}

The overall block diagram of the proposed method is summarized in Figure \ref{fig: supcon}. Within the OLIVES Clinical dataset, each individual image is associated with the clinical values BCVA, CST, and Eye ID that are taken during the original patient visit. For each experiment, we first choose one of these clinical values to act as a label for each image in the dataset. 

Given an input batch of data, $(x_{k}$, and clinical label, $(y_{k}$, pairs $(x_{k},y_{k})_{k=1,...,N}$, we perform augmentations on the batch twice in order to get two copies of the original batch with $2N$ images and clinical labels. These augmentations are random resize crop to a size of 224, random horizontal flips, random color jitter, and data normalization. These are sensible from a medical perspective because they don't disrupt the general structure of the image.
This process produces a larger set $(x_{l},y_{l})_{l=1,...,2N}$ that consists of two versions of each image that differ only due to the random nature of the applied augmentation. Thus, for every image $x_{k}$ and clinical label $y_{k}$ there exists two views of the image $x_{2k}$ and $x_{2k-1}$ and two copies of the clinical labels that are equivalent to each other: $y_{2k-1} = y_{2k} = y_{k}$.

From this point, we perform the first step in Figure \ref{fig: supcon}, where supervised contrastive learning is performed on the identified clinical label. The clinically labeled augmented batch is forward-propagated through an encoder network $f(\cdot)$ that we set to be the ResNet-50 architecture \cite{he2016deep}. This results in a 2048-dimensional vector $r_{i}$ that is sent through a projection network $G(\cdot)$, which further compresses the representation to a 128-dimensional embedding vector $z_{i}$. $G(\cdot)$ is chosen to be a multi-layer perceptron network with a single hidden layer. This projection network is utilized only to reduce the dimensionality of the embedding before computing the loss and is discarded after training. A supervised contrastive loss is performed on the output of the projection network in order to train the encoder network. In this case, embeddings with the same clinical label are enforced to be projected closer to each other while embeddings with differing BCVA labels are projected away from each other.  Our introduced clinical supervised contrastive loss process can be understood by:
$$
    L_{clinical} = \sum_{i\in{I}} \frac{-1}{|C(i)|}\sum_{c\in{C(i)}}log\frac{exp(z_{i}\cdot z_{c}/\tau)}{\sum_{a\in{A(i)}}exp(z_{i}\cdot z_{a}/\tau)}
$$
where $i$ is the index for the image of interest $x_{i}$.
All positives $c$ for image $x_{i}$ are obtained from the set $C(i)$ and all positive and negative instances $a$ are obtained from the set $A(i)$. Every element $c$ of $C(i)$ represents all other images in the batch with the same clinical label $c$ as the image of interest $x_{i}$. Additionally, $z_{i}$ is the embedding for the image of interest, $z_{c}$ represents the embedding for the clinical positives, and $z_{a}$ represents the embeddings for all positive and negative instances in the set $A(i)$. $\tau$ is a temperature scaling parameter that is set to .07 for all experiments.  The loss function operates in the embedding space where the goal is to maximize the cosine similarity between embedding $z_{i}$ and its set of clinical positives $z_{c}$. It should be explicitly stated that the set $C(i)$ can represent any clinical label of interest. Throughout the rest of the paper we will use certain conventions to make the choice of clinical label in the loss transparent. For example, a loss represented as $L_{BCVA}$ indicates a supervised contrastive loss where BCVA is utilized as the clinical label of interest. Furthermore, it is also possible to create an overall loss that is a linear combination of several losses on different clinical labels. This can be represented by: 

$$L_{BCVA + CST} = L_{BCVA} + L_{CST}$$ 

where each clinical value respectively (BCVA and CST) acts as a label for its respective loss. In this way, we are creating a linear combination of losses from different clinical label distributions for the same image. 

After training the encoder with  clinical supervised contrastive loss, we move to the second step in Figure \ref{fig: supcon} where the weights of the encoder are frozen and a linear layer is appended to the output of the encoder. This setup is trained on the biomarker(s) of interest. This linear layer is trained using cross-entropy loss to distinguish between the presence or absence of the biomarker(s) of interest in the OCT scan. In this way, we leverage knowledge learnt from training on clinical labels to improve performance on classifying biomarkers. The previously trained encoder with the supervised contrastive loss on the clinical label from step 1 produces the representation for the input and this representation is fine-tuned with the linear layer to distinguish whether or not the biomarker(s) of interest is present. 




%%%%%%%%% Table shows summarizing statistics across all biomarkers
\begin{table}[]
\centering
\scalebox{.9}{
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{5}{c}{Performance Metrics Averaged Across All Biomarkers}   
\\ \midrule
\multicolumn{1}{|c|}{Method} & \multicolumn{1}{c|}{AUROC} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Sensitivity} & \multicolumn{1}{c|}{Specificity}\\\midrule
PCL  \cite{li2020prototypical}  & $.676 \pm .002$ &  .676 & .572 & .681            \\

SimCLR \cite{chen2020simple}  & $.761 \pm .003$ &  .748 & .591 & .779                  \\
Moco v2 \cite{chen2020improved} & $.737 \pm .002$ &  .734 & .597 & .711                 \\ \bottomrule

Eye ID   & $.802 \pm .001$ &  .769 & .701 & .741                  \\ \hline
CST      & $.793 \pm .001$ &  \textbf{.792} & .601 & \textbf{.803}                   \\
BCVA     & $.801 \pm .001$ &  .785 & .640 & .792                 \\

BCVA + Eye ID   & $.804 \pm .002$ &  .756 & \textbf{.723} & .708           \\

BCVA + CST  & $.807 \pm .001$ &  .783 & .643 & .789               \\
CST + Eye ID  & $\textbf{.819} \pm .001$ &  .756 & .694 & .732            \\

BCVA + CST + Eye ID & $.817 \pm .001$ &  .776 & .677 & .764        \\

 \bottomrule
\end{tabular}
}
\caption{In this table, we obtain the AUROC, Precision, Sensitivity, and Sensitivity across all 5 biomarkers for each contrastive method and then average them together to get a sense of performance across all biomarkers.}
\label{tab:all_biomarker_table}
\end{table}

